Unveiling the Life Cycle of User Feedback: Best Practices from Software Practitioners

User feedback has grown in importance for organizations to improve software products. Prior studies focused primarily on feedback collection and reported a high-level overview of the processes, often overlooking how practitioners reason about, and act upon this feedback through a structured set of activities. In this work, we conducted an exploratory interview study with 40 practitioners from 32 organizations of various sizes and in several domains such as e-commerce, analytics, and gaming. Our findings indicate that organizations leverage many different user feedback sources. Social media emerged as a key category of feedback that is increasingly critical for many organizations. We found that organizations actively engage in a number of non-trivial activities to curate and act on user feedback, depending on its source. We synthesize these activities into a life cycle of managing user feedback. We also report on the best practices for managing user feedback that we distilled from responses of practitioners who felt that their organization effectively understood and addressed their users' feedback. We present actionable empirical results that organizations can leverage to increase their understanding of user perception and behavior for better products thus reducing user attrition.

==> Old_method.tex <==
\section{Research Method}
We conducted an exploratory study on the collection and analysis of user feedback by software organizations.
In particular, we wanted to explore the use of ``social media'' as a source of user feedback to help drive product innovation in software organizations. 
To achieve broader understanding and insights about the state of practice in industry, we adopted a qualitative research design and relied on interviews with practitioners. 
We conducted semi-structured interviews and analyzed the qualitative data to understand the existing industry practice involving leveraging user feedback in software development.  
In Figure \ref{research-process}, we summarize our research process. 
In the following sections, we describe our participant selection, questionnaire design and data analysis methods.  



\subsection{Data Collection}
To answer our interest in how organizations consider user feedback in software development, our first step involved recruiting prospective interviewees for our study. 

\subsubsection{Participant Recruitment and Selection}
To recruit prospective interviewees, we primarily used personal contacts to practitioners working at various positions in software organizations. 
We also relied on networking events and recommendations from other interviewees to increase our pool of interviewees. 
As our study was exploratory in nature we hoped to interview a wide breadth of interviewees who brings a diverse set of experience in collecting or managing user feedback as part of a software development life cycle. 
Hence, we strived to talk with participants who come from a variety of roles, including product managers, chief technology officers (CTO), customer success staff, software engineers, and data scientists. 

We also aimed to talk to practitioners from different sizes of organizations as the size could play a role in the practices and challenges experienced by an organization.
According to the OECD,\footnote{https://data.oecd.org/entrepreneur/enterprises-by-business-size.htm} a small business has less than 50 employees, a medium business has between 50 and 249 employees, and a large businesses has 250 or more employees. 
We did not solely study large organizations, who likely have more resources than smaller counterparts and are likely using the best practices for managing user feedback. 
As small and medium sized organizations represent the vast majority of businesses,\footnote{https://www.worldbank.org/en/topic/smefinance} we felt our approach would help uncover discrepancies between the organizations and identify potential areas of improvement.  
Additionally, we strived to talk to practitioners from a wide range of industries to help fill the breadth understanding. 
Our study participants come from software organizations that pertain to industries ranging from financial, e-commerce, content provider, and gaming. 
We recruited participants into our study until reaching thematic saturation \cite{cruzes_recommended_2011}. 

We had a few basic selection criteria for our interviewees which included:
(1) involved in user feedback collection (e.g., customer success agent who takes user phone calls) and 
(2) involved in feature development life-cycle in some capacity (e.g., product manager who makes final decision to add a new feature).

\subsubsection{Interview Design}
We conducted 40 semi-structured interviews that required approximately 30 to 60 minutes of each participant's time. 
Table \ref{demographic-table} provides the demographic details of our participants. 
In total we interviewed forty participants from thirty two organizations.
Among them we had participants from nine small, nine medium and fourteen large organizations.

The semi-structure, interview questions were prepared by the research team following the \textit{general interview guide} method \cite{patton2002qualitative}.
We started each interview with introducing the intention of the research to the participants and asked them to start with discussing their roles and responsibilities at the company. 
We followed the base interview transcript for each interview which includes questions such as \q{What is a typical process for your company to identify features to develop? What is your feedback loop, who is involved in the feedback and release process? What are the challenges that you've experienced collecting user feedback? What social media sources do you collect to understand user concerns?}. 
We provide our base questions in the replication package. 
Although the questions mostly revolved around these questions, occasionally we added questions relevant to their specific roles or situation so we improvised depending on the participants response.  
For each interview, detailed notes and recordings of were taken for our subsequent data analysis step. 
The recordings of the interviews were later transcribed which allowed us to thoroughly analyze the data. 


%Write the P and O number

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h!]
\centering
\setlength\extrarowheight{-10pt}
\small
\begin{tabular}{@{}llp{3.4cm}p{1.2cm}p{1.8cm}@{}}
\toprule
\textbf{Org.} & \textbf{P\#} & \textbf{Role} & \textbf{Org. Size} & \textbf{Industry}\\ \midrule
O1 & P1 & Co-Founder and COO & Small & Analytics \\ \midrule
O2 & P2 & Founder and CEO & Small & Analytics \\ \midrule
O3 & P3 & Founder and CEO & Small & Analytics \\ \midrule
O4 & P4 & Product Manager & Small & Educational \\ \midrule
O5 & P5 & Software Engineer & Small & Crypto \\ \midrule
O6 & P6 & Co-Founder and CTO & Small & Food SaaS \\ \midrule
O7 & P7 & Co-Founder and CEO & Small  & Financial \\ \midrule
O8 & P8 & Head of Engineering & Small & CMS \\\midrule
O9 & P9 & Senior Product Manager & Small & Healthcare \\ \midrule
\multirow{3}{*}{O10} & P10 & Cust. Success Manager & \multirow{3}{*}{Medium} & \multirow{3}{*}{E-Commerce} \\
 & P11 & Data Analyst &  \\
 & P12 & Product Manager &  \\ \midrule
 O11 & P13 & Cust. Success Manager & Medium & Content \\ \midrule
 O12 & P14 & Co-Founder and CTO & Medium & Food SaaS \\ \midrule
\multirow{2}{*}{O13} &  P15 & Technical Lead &\multirow{2}{*}{Medium} & \multirow{2}{*}{Analytics}  \\
 &  P16 & Co-Founder and CTO & \\ \midrule
O14 & P17 & QA Engineer & Medium & Content  \\ \midrule
O15 & P18 & Software Engineer & Medium & Healthcare \\ \midrule
O16 & P19 & Data Engineer & Medium & Music \\ \midrule
O17 & P20 & Backend Engineer & Medium & Dating \\ \midrule
O18 & P21 & Software Analyst & Medium & Industrial SaaS \\ \midrule
O19 & P22 & Senior Engineer & Large & Automobile \\ \midrule
O20 & P23 & Product Manager & Large & Travel \\ \midrule
\multirow{3}{*}{O21} & P24 & Software Engineer & \multirow{3}{*}{Large} & \multirow{3}{*}{Software} \\ 
 & P25 & Senior Product Manager &  \\ 
 & P26 & Software Engineer & \\ \midrule
\multirow{3}{*}{O22} & P27 & Product Manager & \multirow{3}{*}{Large} & \multirow{3}{*}{E-Commerce}  \\
 & P28 & Software Engineer &  \\ 
 & P29 & Software Engineer &  \\ \midrule
 O23 & P30 & DevOps Engineer & Large & Security SaaS \\ \midrule
O24 & P31 & Data Engineer & Large & Insurance \\ \midrule
O25 & P32 & Software Engineer & Large & Gaming \\ \midrule
O26 & P33 & Data Scientist & Large & Financial \\ \midrule
O27 & P34 & Software Engineer & Large & MaaS \\ \midrule
 \multirow{2}{*}{O28} &  P35 & Head of Consumer Product &\multirow{2}{*}{Large} & \multirow{2}{*}{Software}  \\
 &  P36 & CTO & \\ \midrule
O29 & P37 & Requirements Engineer & Large & Technology \\ \midrule
O30 & P38 & Technical Project Manager  & Large & Gaming \\ \midrule
O31 & P39 & Data Engineer & Large & Social Media \\ \midrule
O32 & P40 & Senior Software Engineer & Large & Advertising \\ \bottomrule
\end{tabular}
\caption{Participants and Their Roles and Organizations}
\label{demographic-table}
\end{table}



\subsection{Data Analysis}
The analysis process comprised of few different steps.
As we recorded each interview, we transcribed them using an automated transcribing tool that converted the audio to text.
We utilized thematic analysis \cite{cruzes_recommended_2011} to identify the initial codes from the raw data related to industry practices for utilizing user feedback in their software development process.  
To minimize any bias, an open coding approach \cite{corbin1990grounded} was adapted to identify patterns.

Two of the co-authors pair coded the interview transcripts until a shared understanding on the codes was reached. 
This shared understanding was reached after six rounds of pair coding.
The respective Cohen's Kappa \cite{landis1977measurement} for the six rounds were 0.51, 0.72, 0.73, 0.88, 0.76, and 0.76 which indicates we had a substantial level of agreement.
After each pair coding session, the two co-authors would discuss the definition and usage of the codes to increase shared understanding. 
Subsequently, the two co-authors proceeded to individually codify the remaining thirty-four interviews.
During individual coding, another co-author would conduct a sanity check through the coded transcript to catch potential missing codes or incorrect labels.  
Our coding process resulted in 42 codes that were reviewed and refined by the co-authors.
In our next step, we developed themes from our coded data and the main points of each quote by discussing the similarities and differences of the codes and main points and congregating into themes that answer our RQs.

For example, the \textbf{raw quote:}, \textit{``If it's [affecting] the ability for somebody to log into their email, just as an example, [we] don't need to look at data to know that that is a high priority, kind of a showstopper issue, and it needs to be addressed immediately. That's where we'll lean on data to help us decide what to prioritize now,"} consisted of the codes  Prioritizing, FeedbackfromSoftwareUsage, MethodsToAnalyzeTrends, IdentifyingTrends.
This helped us find the underlying main point of the quote which is how organizations prioritize user feedback and the theme \textbf{Prioritizing User Feedback}.

\subsection{Member Checking}
\nowshin{Add Member checking}


In the next few sections, we provide an in-depth analysis of our exploratory study and our conversations with our participants.
We highlight the key findings about managing user feedback, particularly the social media aspect and what it means to be high a functioning organization for user feedback.
We also discuss the differences and similarities identified in our study where relevant with previous literature about product management.

==> old_findings.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%Findings from March 25

\section{Results}
% User feedback is a highly critical aspect for software organizations to consider as part of building new features and resolving bugs.
% Social media user feedback, a growing segment of user feedback, has great potential to influence user behavior, which may in hindsight impact whether users continue using a software \cite{li2022narratives, voramontri2019impact}. 
% Despite the efforts of various studies to learn about the use of user feedback in the industry \cite{van2021role, johanssen2019practitioners}, there is still a lack of empirical evidence on the best practices for utilizing user feedback, especially social media feedback, in product management. 
% To address this, we embarked on this study with the goal of reaching out to industry practitioners to gather insights on whether software organizations even consider social media user feedback and if they \textbf{do} consider social media, what are the actions they exercise to manage these user concerns.
% Our 40 interviewees from 32 organizations confirmed that understanding user concerns, especially from social media, is critical to their product management.
% Our interviewees also highlight the perils of not considering or misunderstanding these user concerns.

% Preview findings, briefly describe the life-cycle and the factor. 

Our research delves into two fundamental concepts that emerged from analyzing the feedback of 40 interviewees from 32 organizations.
We start by discussing the importance of user feedback in organization and the degree to which it influences their product development. 
We then describe the life-cycle to manage user feedback based and factors that make an organization high performing for managing the user feedback.
Our findings are based on the interview analysis and existing literature.

\subsection{Setting the Scene: Why User Feedback Matters Greatly to organizations}
\emph{Consequences of Misunderstanding User Feedback:}
A common theme that emerged throughout our interviews with practitioners was the criticality of \emph{accurately} understanding user feedback.
They reinforced the dangers and consequences of misunderstanding user feedback, especially social media, as this can lead to misguided decisions and wasted resources.
P1 used a movie example as an analogy to illustrate the potential consequences of misinterpreting users on social media. 
\qs{The movie Morbius became a meme... The core of the meme was that no one had actually seen this movie. [Discussion on social media] became very popular. Sony actually extended the theatrical release of the movie, because they saw a trend that the popularity of the movie was increasing. They did not test to determine that the reason why the popularity of the movie had increased is because people were having fun talking about how no one had seen or any intention of seeing the movie.}{P1} 
The result was that the company wasted the money re-releasing and re-marketing the movie to no audiences \cite{mendelson_box_morbius}. 

P1's example about Morbius touches on two crucial aspects regarding social media user feedback. 
First, social media user feedback snowballs and can increase in magnitude so organizations should consider it \cite{arif2016information}. 
It would be in the interest of an organization such as Sony to consider the discussion and potentially harness the discussion to its benefit.
Second, consequences of misunderstanding social media feedback is costly.
If Sony made an accurate assessment of user feedback, they would have realized that no one would spend money on the product, but their attention was just on the pure volume of mentions of the movie.
Hence, our participants emphasized that it's not enough to just consider feedback, they also need to accurately assess user feedback to understand what is influencing user perception regarding their product. 

%\subsection{
\emph{Influencing User Perception:} 
% Due to the ease of communication, user feedback on social media can easily travel to other users.
% Consequently for software organizations, user perceptions related to a software product can suffer from sudden trends in user concerns \cite{li2022narratives}.
% For example, some software products have widely been reported to suffer from a perceived lack of privacy and transparency on social media and in turn users have flocked to competing platforms during the turbulence \cite{li2022narratives}. 
Software products have widely been reported to suffer from a perceived lack of privacy and transparency on social media and in turn users have flocked to competing platforms during the turbulence \cite{li2022narratives}. 
In this study, participants also highlighted the role that user perception plays on user behavior.
As exemplified by P35 \q{if you think about user behavior in certain patterns, it also spurs research and insights and feedback to a large degree, you know, because you can take that and mold it and shape it and put it back into a product road map.}

In other words, when a user struggles to even understand the main features of a software, it is likely that users will complain or refuse to use the product.
User complaints is still problematic because the organization will still have to address them to diffuse negative concerns.
% Therefore, our participants emphasis the need for influencing user perception.
% In addition to accurately recognizing and assessing user perceptions, organizations should actively shape perceptions around their software.
% For example, O12 receives a consistent stream of user feedback on social media spaces where users would criticize O12's software for lacking features that competitors provide.
% This is a constant challenge for O12, which they have to continuously monitor social media and dissuade the user perception that they lack features.
% They explained to us that these ``missing features" are not possible for them nor competitors as they are all limited by the same technology.
% To this end, O12 has to manage the user perception and educate users about the reality.
P31 explained the measures that their organization took to increase the positivity from user perception on social media.
\q{[We] used to analyze the perception. So most of the times the feedback is negative on Twitter. [Redacted] made efforts to improvise that image in public by analyzing the tweets and then taking action.}
Upon releasing new features to users that addressed major concerns, the number of negative feedback decreased. 
The reduction in negativity in user perception was a result of carefully curated efforts to increase positive vibes by delivering features well received by users.


% Recall that understanding the ``voices of users" and the user perception often trending on social media are necessary for software organizations.

The consequences of not acting or acting wrongly on the user feedback and perception are both significant and best avoided.
To identify practices to manage the the user feedback, we conceptualize and propose a novel user feedback data-flow pipeline (Figure \ref{voice-of-users-data-flow}) for software organizations based on our interviews with industry practitioners and previous literature.
% We describe these practices in detail in the next subsection.

% \qs{If we were to only build on our vacuum we will only do what we think we need. We're missing out on the experiences and the needs of others. ... Otherwise, you're going to build what you want. And you're going to miss probably 99.9\% of what everybody else wants, right?}{P35}

% Users frequently post feedback on various platforms with the expectation of a response from organizations.
% Ideally, an organization will address the feedback through a future iteration where a feature or bug is resolved according to the feedback.
% However, users often have a limited perspective and may not fully comprehend the resources and limitations of software organizations.  
% \qs{customers kind of exist in their own bubble, they never think about other customers, it's always it's a problem for them.}{P11}
% On the other hand, organizations must strive to identify the most relevant feedback that is aligned with their company's goals and values.


% While user perception is important to manage, it is a difficult task because on social media \qs{there are people who are louder than others}{P12}.
% Louder voices could dampen other voices and may not represent the entire user base.
% I'll think about it. Yeah. I mean, I will say as well, though, and this is just, you know, from the experience of working in, you know, open source intelligence and social media analytics. It's not a thing that most like, groups that even do it do well, like, it is so easy to confirm your bias with social media data or to, to sort of to find, like incorrect conclusions. 
% I think it is, it is very rarely done in a way that would even approach scientific. So, you know, I don't think we're yet at the point where, you know, industry standard or even industry best is, you know, what I'd call like, scientifically good. That's, that's really just genuinely where we're at right now.

% Why you combine two concepts, why you split the sources into 3 categories. 
% stress the importance of social media
% reason of splitting: some org don't use social media but they dont have resources. but conventional ways anyone can do it. anyone can do it.  
% Socail media is new, challenges but this why we classify it.
% The way you analyze use metric is different
% Quotes from interview: dangers of social media P1. echo chamber.
% In the conventional ways: they are straight forward
% Social media: get more feedback but there's more noise. 
% P14 say user metric is hard to analyze becase they dnt wanna hire anyone. 

\subsection{Managing User Feedback}
\subsubsection{Collection of User Feedback}
The first critical aspect to managing these user feedback is identifying where and what to look at. 
Our participants expressed a significant variety of sources of feedback important to their business that we list in Table \ref{tab:user-feedback-sources}.
In particular, vast majority of organizations \org{1-2, 5, 11-27, 29-31} discussed the importance of collecting \textbf{social media} user feedback to understand issues and needs of the product.
\qs{We have a team that just looks at social media [feedback], and they report on the biggest trends coming from social media.}{P27}
We noticed in our interviews that organizations are increasingly considering social media feedback, especially from newer types of social media such as TikTok \org{17, 25}, Discord \org{1, 2, 5}, and Instagram \org{1, 17, 20, 31}.  
While previous studies on user feedback have tried to provide greater understanding on the types of feedback, they did not specify the details on how organizations actually collect and utilize the social media feedback \cite{van2021role}.

We found that large organizations often paid close attention over social media, which is reasonable as they typically generate a lot of media attention.
\qs{You can imagine this company is in the news all the time. It's definitely a part of our weekly life of what we look at.}{P27}
In contrast, we found that many smaller organizations do not consider social media as they have not reached the scale to experience a large magnitude of feedback \org{3, 4, 6, 7, 9}.
Our finding contradicts earlier research on the proliferation of user feedback in organizations, which indicated that small organizations consider social media, where as large ones do not \cite{10.1145/1984701.1984702}.

However, the smaller organizations that do consider social media in our study have extensive experience and shared some the pitfalls and mitigation strategies.
For example, both O1 and O2 heavily rely an assortment of social media to build understanding of the user base and conceptualize new features.
\qs{Before we jump in and spend \$40,000 plus on developing that functionality... let's get a sample of the social media posts, let's get a sample of the events in question.}{P1}
The pitfall of confirmation bias is non-negligible, \qs{if you are looking for something in social media, you will find it right, like the ability to determine like confirmation bias and social media is pretty, pretty fantastically high.}{P1}
Acknowledging that there could be bias on social media, P2 shares a practice they use to reduce bias in their data collection.
\qs{I ask questions [to the community]. Generally I don't ask question under my name. I have some fake names that I use. So I have some fake name with a male and a female account. [One] needs to stop being biased. Some guys want to seduce a girl and some guys are gonna be aggressive with us. So I'm basically trying to have neutral data points, non biased, you always going to have bias, but your goal is to reduce bias.}{P2}
In other words, successfully managing user feedback, especially from social media, starts with collecting non-biased user feedback from users.

In addition to social media, our participants mentioned numerous other sources of feedback such as user workshops, app reviews, and community forums. 
These sources have long been used as part of product management and collecting user feedback, which is in line with previous studies in this area \cite{van2021role}.
However, our participant interviews revealed another divergence from previous literature regarding the categorization of sources of user feedback.
Maalej \emph{et al.} \cite{maalej2009users} categorize user feedback into two types: explicit and implicit feedback. 
Explicit feedback is the feedback that users provide directly through different channels, such as app reviews, while implicit feedback is unintentional feedback from users, such as through software usage metrics.

In contrast, based on interviews regarding how organizations \emph{collect} and \emph{manage} feedback, we split the various user feedback channels into 3 broad categories as shown by Table \ref{tab:user-feedback-sources}: social media, conventional, and user usage metrics.
We found that depending on the feedback channel (i.e., social media, user metric, etc.), the organizations manage them quite differently.
This difference largely originates from the original provenance of each user feedback.
After all, for conventional user feedback, a user is providing direct user feedback to a particular software organization in the form of a phone call, video conferencing, or user workshop.
Regardless of the form of conventional user feedback, an organization receives feedback from someone who is likely using of the product.
For social media feedback, a user typically provides feedback in the form of video (e.g., YouTube or TikTok) or textual (e.g., Twitter or Facebook), but the feedback may or may not be from an actual user.
Sometimes, social media feedback is more amplified due to the fact that \qs{if someone starts talking about a particular feature, more people will start talking about that feature, that doesn't necessarily mean that is a valid signal, they're talking about it because of conversation is occurring}{P1}. 
Recall, the example with the movie Morbius, people mentioned the movie on social media, but the movie studio had no way to know if these people were actual moviegoers or not.
We found that organizations treated the two types differently as with conventional user feedback, the organization was often talking or observing a verified user.
In comparison, a social media user does not necessarily refer to a real or even potential user.
The amount of data between the two categories also vary greatly, where there is a likelihood that the volume of social media data is much greater than conventional user feedback.

Finally, we categorize data collected by tools such as Hotjar or Google Analytics in the category user usage metrics.
These tools are sophisticated enough so that anyone at the software organization could replay a user usage session like a movie and visualize every button click, mouse hover, and delay on page. 
\qs{Everything is tracked, every click is [tracked], every action is tracked. That user feedback is how users interact with the [product].}{P39}
With user usage metrics, an organization receives a source of feedback that accurately represents user actions and does not depend on what users are telling the organization.

Essentially, an organization collecting conventional feedback will most often acquire textual transcripts of user input from sources like support tickets and emails. These sources will also often include photos or screenshots of the software, which organizations will collect into issue tracker systems.
Similarly, social media feedback is also often collated in the form of text or image, but social media requires a lot more active monitoring and this process for monitoring is very much ad-hoc.
Important feedback eventually gets added to issue tracking systems as echoed by P19,``We have different Jira [projects]," Jira ticket is created when ``someone [on] feedback collection team collect some requirements or feedback.
User usage metrics often plays a supporting role in validating the two other types of feedback. 
\qs{People tweets, right? So there are different channels they [talk]. Our product managers monitor those channels. [Redacted] is a live game if something is impacting the people they complain in those channels. And we see that. We will align people complaining that they cannot log in with our graphs and charts [user usage metrics].}{P32}


% \kezia{there might be some repetition here between this paragraph and the intro and sec 2.3} 
Based on our interviews, we realized that there are various channels of ``voices of users" that organizations should consider. 
% To encapsulate all the channels, we borrow the concept coined by Tizard \emph{et al.} \cite{tizard2022voice, tizard2020voice} regarding ``Voices of the Users.''
% , which they refer as the collection of user feedback and opinions expressed through various channels, informing software organizations of their needs.
From previous literature we group ``voices of users'' by reorganizing the various sources into three categories mentioned in Table \ref{tab:user-feedback-sources}.
The three types of user feedback is collected and processed in different ways resulting in our categorization into three types. 
Our approach is meant to help industry practitioners learn the most effective ways to manage each type of user feedback.

 

\begin{table}[h!]
    \centering
    
    % \setlength\extrarowheight{-10pt}
    \small
    \begin{tabular}{p{1.35cm}p{2.5cm}p{3.5cm}}  \toprule
    Category & Source & Organizations That Heavily Rely On This Source\\ \midrule
    \multirow{9}{*}{Social Media}   & Reddit & 1-2, 12, 16-17, 19, 21-22, 25, 30 \\ 
    & Twitter  & 1-2, 5, 11, 13, 17-18, 22, 24-26, 29-30 \\ 
    & YouTube & 1, 23, 30 \\ 
    & Discord & 1, 2, 5 \\
    & LinkedIn & 7, 12, 21, 23, 29 \\
    & TikTok  &  17, 25 \\ 
    & Instagram  & 1, 17, 20, 31 \\ 
    & Facebook & 17, 19, 27, 31 \\
    & Community Forums & 4, 6, 8-12, 18, 21, 22, 30, 31 \\ 
    \midrule 
    \multirow{6}{*}{Conventional}    & Email  &  1-32 \\ 
        & Phone Call  &  3, 4, 6, 7, 9-11, 16, 22, 25, 28, 30 \\ & Video Conferencing & 3, 4, 7, 20 \\ 
        & Support Channels & 1, 4, 5, 9, 10, 11-25, 27, 28, 30-32
        \\ 
        & App Reviews & 17, 22, 25, 26, 27, 28, 30, 31 \\ 
        &  User Workshops &  11, 28, 29, 30 \\ \midrule
        User Usage Metrics & Data from Tools (e.g. Hotjar, Pendo, Google Analytics, etc) & 1-8, 10-11, 13-14, 16-17, 19-23, 25-31\\
        \bottomrule
    \end{tabular}
    \caption{User Feedback Sources}
    \label{tab:user-feedback-sources}
\end{table}



\subsubsection{Analysis of User Feedback:}
Our participants indicated the next step after collection is analyzing the trove of feedback.
We found that organizations heavily rely on manually looking through incoming user feedback to uncover underlying patterns and trends received through all 3 categories of user feedback sources.

%theme identifying process for both social media and conventional
Key to the process is listening to the bastion of user voices and group similar patterns.
\qs{What are the things that they struggle with. [We] went through all that feedback and grouped the similar themes about what were the common complaints and and what were the common dream features that everybody wanted.}{P4}
The same question repeated again and again is often representative of a underlying problem. 
\qs{The number of times the question was raised was also important, because that means many [users] are having this confusion.}{P5}
When customer complains through support channels, the volume of complaints can illustrate trends as well.

\begin{wrapfigure}{l}{0.12\textwidth}
  \centering
    \vspace{-10pt}
  \includegraphics[width=0.16\textwidth]{figures/analysis.pdf}
    \vspace{-20pt}
  % \caption{User Feedback Triangulation}
  \label{validation}
\end{wrapfigure}

%indicating that the analysis process is somewhat same but differs in reliability
For both conventional and social media user feedback, organizations tend to consider a topic as a ``theme'' when it gains traction. 
However, they may view the information presented through conventional sources as more credible, as social media feedback may be more noisy.
In the case of user usage metrics, organizations look for patterns through the graphs that indicate a trend. 
As described by P10,\q{ Pendo is kind of cool. Because it tracks every click, you can go into it on a user level and see exactly where someone clicked, at what time, and they generate these fantastic graphs for you that say, you know, this person spent 80\% of their time on this one.} 

%What happens to the generated themes. How themes are sent to next phase.
Once the common ``themes'' are generated, they are sent to the next phase through different methods such as Jira tickets.
\qs{Once we have kind of enough information, like enough background of what the root issue is ... who is it's going to affect? Is it affecting every user, how big of a deal is this? The product team creates a [Jira] ticket ... literally just mentioning the issue, ... and then we work on it and scope it out and do our research that is needed. And then yeah, it is forwarded from there.}{P4}

%How social media is a good addition to the data
The perks of using social media user feedback includes rapid insights on bugs that occur in the product.
\qs{During the testing process. We missed [including the menu items]. We woke up one day... All these messages on social media being, ``what the heck, I just updated and none of the menu items [exist] anymore." }{P13}
We see the importance of pure volume of feedback manifesting as a key factor of identifying themes.
\qs{People will post snapshots of a Reddit post with a whole bunch of votes. And [users are]  mad about the [feature], or on the new UI. And then a month later, there's a JIRA ticket and someone's working on it.}{P22} 


A challenge with this approach is the presence of noise, particularly in social media where spontaneous comments can quickly gain momentum. 
P38 points emphasizes that it's essential to balance the signal-to-noise ratio and consider which groups of users are over-represented or under-represented in this type of feedback. 
After all, some groups may be more likely to post on social media than others, which can skew the data. 
It's important to ensure that the feedback received represents a diverse range of users and is not biased towards any particular group.
Users may also have conflicting opinions or report pain in the spur of the moment.
\qs{A lot of the time, requests come in, they're not flushed out fully. In the moment, they're frustrated with something. And then two hours later, [they] don't need that.}{P14}
It is crucial to listen to all feedback, but it is equally important to recognize that not all feedback is equal.
Oordt and Guzman \cite{van2021role}, reported practitioners echoing similar concerns about ``feedback quality'', as many times they are ``noisy'' or lack overall ``representativeness''. 

The process of analyzing social media content is predominantly carried out manually by individuals or teams who actively monitor social media platforms during their regular activities. 
Many of the successful companies have teams that conduct this analysis.
However, smaller companies struggle with the process and prefer to have a tool that would support their team. 
This is in line with previous research by Oordt and Guzman \cite{van2021role}, where they reported that industry practitioners tend to incline more towards manual analysis methods.

Their study further revealed that that there was limited usage of automated feedback analysis among industry practitioners, despite a significant number of tools developed \cite{carreno2013analysis, guzman2014users, iacob2013retrieving, maalej2015bug, oehri2020same, panichella2015can, gao2022listening}. 
Our participants reported similar limitations but also specified the reasons why they do not rely on these tools.
The existing tools are either too hard to use, expensive or still not publicly available for them to use.  
For example, O4 attempted to use an existing tool to analyze their community forum in a better way. 
However, they realized that the tool was not as effective as expected and had an expensive yearly subscription cost (20 thousand dollars/year).
Hence, our findings indicate there is high emphasis on identifying reliable ``themes", albeit through manual analysis, there is strong demand for tools that can enable reliable and cost efficient feedback analysis. 



\subsubsection{Validation of User Feedback:}\label{sec: validation}
One important aspect of the user feedback pipeline is the validation of emerging ``themes" that arise from the analysis phase. 
Validating user feedback is an important process with the end goal to mitigate misinterpretation and misunderstandings.

\begin{wrapfigure}{l}{0.12\textwidth}
  \centering
    \vspace{-10pt}
  \includegraphics[width=0.16\textwidth]{figures/validation.pdf}
    \vspace{-20pt}
  % \caption{User Feedback Triangulation}
  \label{validation}
\end{wrapfigure}

The validation process involves triangulation between the 3 categories of user feedback to reduce misinterpretations.
\qs{In theory, if a [social media] trend is significant, you should be able to see the impact of that trend in your own user observation data as well. And if you can't, that's either you're not doing very good user observation data, or the trend is not impacting you yet.}{P1}
One can compare the themes from conventional and social media sources with user usage metrics and vice versa. 
Another possible strategy is starting with social media to identify themes and then directly contacting users to validate. 
\qs{Social media is a good place to get started. You find a trend. Next step is to collect a statistically relevant, smaller sample of genuine accounts that you care about.}{P1}
After this process, an organization would have ``collated a list of feature and bug concepts'' that were validated and represent genuine issues. 


By tracking user engagement with different tooling such as Hotjar or Google Analytics, we can see which features are being used effectively and which ones are being ignored. 
Social media on the other hand come with a lot of noise as discussed previously, but triangulating the themes from social media with user metrics can help understand the user behavior better.
\qs{Feedback is a gift... The metrics don't lie. Metrics are metrics, they have no face... Sometimes it's about how a new feature or change you made, sometimes it's about a bug, you always look for what's the cause and effect of a change in a metric. So you have to kind of look at it from that aspect and realize that you can't always get [feedback] from direct comments from users. That always works out really well.}{P36}
A study suggests that industry practitioner rarely applied systematic validation of user feedback \cite{johanssen2019practitioners}. 
While existing literature adds various feedback collection, analysis, and prioritization processes in depth \cite{van2021role, seyff2017end, firesmith2004prioritizing, gartner2012method, johanssen2019practitioners}, there is a dearth of discussion on how to determine the validity of the emerging ``themes". 

% \nowshin{Find a better inter team coordination quote related to validation}
% A possible solution, identified from an existing study by Seyff \emph{et al.} \cite{seyff2017end}, suggests having a ``designated decision maker'' (e.g., a product owner) to review feedback from various channels, prioritize requirements, and validate them to some extent. 
% However, the ``designated decision maker'' would also need to coordinate with other departments to fully leverage the validation process.

Establishing tools and processes to support this triangulation could be another possible solution.
This effort is worthwhile for organizations as it increases the likelihood of identifying which features and bugs are relevant and impactful for users before investing valuable engineering and product hours.
Especially, in this era where there are multiple sources of user feedback that organizations have to take into consideration. 


\subsubsection{Prioritization of Requirements}
Our interviewees highlighted that prioritization is a crucial step in the life cycle to manage user feedback, which involves making trade-offs between different bugs and features to maximize benefits for the organization. 

A critical factor to prioritization indicated by our interviewees is whether the `collated list of feature and bug concepts'' received from the validation stage match a company's vision and goals. 
Best described by P27, \q{if we get feedback, that doesn't align to anything we're doing.. [if] it's not something that we're going to address this year, we're not going to redesign it, we're not going to revamp it.}
That is not to say that they would completely ignore it, \qs{I'd probably look at little quick fixes I could make.}{P7}

\begin{wrapfigure}{l}{0.12\textwidth}
  \centering
    \vspace{-10pt}
  \includegraphics[width=0.16\textwidth]{figures/prioratization.pdf}
  % \caption{User Feedback Triangulation}
  \vspace{-20pt}
  \label{validation}
\end{wrapfigure}

Furthermore, the underlying driving force for major features is often the revenue that a prospective feature may bring to the organization.
\qs{We need to make money. If there is a feature that one customer wants and [has] a significant impact on revenue, we're going to implement [it]. [The] features need to be reasonable. If they ask to put a pink elephant on the homepage, we're not gonna do that. But if they implement a feature that's gonna benefit [many] people. Yes. We're gonna do that. But it needs to drive revenue.}{P2} 
Organizations place emphasis on activities that generate revenue or prevent financial losses, while also factoring in practical considerations.
This is in accordance with existing literature \cite{berander2005requirements, sivzattian2001linking} where cost and risk have been indicated as major aspects of requirement prioritization. 

The key to prioritization is balancing trade-offs so that there is mutual benefit for the users and organization. 
P6 astutely observes, ``if they [users] are giving us [feedback], it's likely...that [something] would help them. [They] help us because they are going to use our system."
Our participants further reported user perception as a crucial factor in the prioritization phase. 
As P28 participant pointed out, \q{people's perception of the company as a whole} is also an important factor. 
If the feedback is related to something that is damaging the company's reputation, it will be given priority even if it doesn't have a direct financial impact. 
After all, a company's reputation is invaluable and can influence user behavior to adopt or drop a software product \cite{li2022narratives}.

Our participants also described that they most often prioritized bug fixes over features. 
Bugs are almost always prioritized over feature requests as bug indicate a blocker to current revenue, a top priority issue, where as new features is usually meant to obtain future revenue.
\qs{New features are typically lower priority than bug fixes. So usually bug fixes are prioritized top of the list, because it's something that the users are paying for or having issues with as compared to something that just doesn't exist.}{P17}


Not all feedback is created equally and the often ad-hoc process of prioritizing can result in the wrong decisions, which is particularly troublesome for smaller organizations with limited resources. 
\qs{Sometimes we end up choosing such a [feedback] to implement, which probably just takes a lot of time. [Alternative] task which [ended up] more important gets delayed. So we do make mistakes, but we try to avoid that by discussing and analyzing.}{P6}
There have been multiple approaches suggested to aid in the process of determining the priority of requirements \cite{achimugu2014systematic, firesmith2004prioritizing}. 
A number of studies have focused on automating the end user feedback prioritization process \cite{licorish2017attributes, kifetew2021automating, gartner2012method, malgaonkar2022prioritizing, gao2022listening}, however as reported by our interviewees, industry practitioners rarely utilize the tools.  


Prioritizing user feedback is a necessary step that requires balancing trade-offs for features and bugs.
By striking this balance, an organization may create software that not only meet user needs but also align with their larger vision and goals.

\subsubsection{Development of Feature Request and Bug Fix}
At this point, an organization has identified initial themes based on user feedback, developed feature or bug concepts through validation, and prioritized the important features or bugs.
The last step of the life cycle to manage user feedback is the development and eventual release of new features or bug fixes from an organization's prioritized list.
This is when the technical team is given the most responsibility to develop the software to match user requests. 
When an organization finishes development and the new version of the software passes all assigned tests, the organization will release the software to its users at the next opportune time.
% Depending on the organization, this interval could range from minutes to months. 
However, when that new software version is released to users, a new cycle of the life cycle to manage user feedback is triggered and new user feedback, good or bad, will makes its way to product managers, developers, customer support staff, data scientists alike. 


\begin{table}[!t]
    \centering
    \small
    \begin{tabular}{p{2.0cm}p{5.7cm}}
        \toprule
       \textbf{Factors}  &  \textbf{High Performing Criteria} \\ \midrule
        Active Employee Participation  & Every employee is actively contributing to the life cycle to manage user feedback (i.e., collection, analysis, validation, and/or prioritization) \\ \midrule 
        Active Feedback Collection &  
        Proactive data collection from all the feedback sources related to the product.  (i.e., Sources equal \emph{n} where \emph{n} is number of sources containing an organization's feedback and $\emph{n}\geq$2 )
           Sources must come from at least 2 out of 3 feedback categories \\ \midrule
       Active \par Triangulation\strut   & Organization actively leverages 2 or 3 categories (i.e., social media, conventional, and/or user usage metrics) to validate the ``collated list of bugs and features'' \\ \midrule
       Active Response  & Prompt response to the feedback. Response could be in terms of marketing, communication and/or bug fix or feature roll-out.  \\ \bottomrule
    \end{tabular}
    \caption{Factors For High Performing Organization for Managing ``User Feedback"}
    \label{tab:high_performer}
    \vspace{-15pt}
\end{table}




\subsection{Factors to Become High Performing at Managing User Feedback}
From our interviews with the industry practitioners, an emerging theme has been a set of best practices that our interviewees utilize to most effectively understand and respond to user feedback.
Many participants were eager to share with us the best practices they utilized to achieve good understanding of users, which they described made them feel confident about their ability to address user needs. 
We contextualize these best practices as factors that organizations may consider to become a "High Performing Organizations" for managing ``voices of users."
\zane{Maybe something here about previous work in defining high performing organization?}
Other participants indicated it would be beneficial for them to learn about the best practices. 
As echoed by P6, \q{And especially, you know in startups, because the real struggle is we don't know the best practices out there.}
Based on our interviewees, effectively managing "voices of users" can lead to increased customer satisfaction, expedited product deployment, and ultimately, higher revenue for software organizations.

For an organization to be high performing, they need to fulfill four factors that we refer to as the \textbf{4A}s: 1) active employee participation, 2) active feedback collection, 3) active triangulation, 4) and active response time. 
Table \ref{tab:high_performer}, indicates the \textbf{4A}s and the criteria to satisfy each criteria.  
% In the following section, we describe how organizations can accomplish the \textbf{4A}s based on our findings.


\subsubsection{Active Employee Participation} \label{sec: active employee participation}
High performance starts with an environment that encourages employees to thrive in the product feedback management.
More specifically, when employees in different management and development roles actively participate in the feedback collection, analysis, validation, and prioritization, the team can effectively incorporate feedback from all three categories of "voices of users". 

We found that large organizations \org{O19, O21, O22, O27, O31} often heavily encourage their employees to take the initiative, particularly for identifying issues in the software products.
\qs{There's a lot of ownership among devs. If you're working on something, it's expected that you own that and see the potential risks and impact of you're doing and make design decisions for that.}{P22}
Employees who are invested in the product may pick out themes in user complaints on social media while browsing,
\qs{High majority of [redacted] employees are also very interested in [redacted]. It's very common that the employees will frequent [redacted]'s subreddits. [Some] bug reports and feedback comes from internal employees being on [redacted] related social media.}{P22}
Therefore, employees frequently will post screenshots from social media regarding popular concerns that impact the product \qs{[We see] screenshots of a Facebook post saying ``what does this alert mean?" And then someone's on it, trying to make the customer facing UI more understandable or adding something to the user manual. This \textbf{initiative} is definitely led by employees that have other jobs that just happen to be also invested in these kinds of things.}{P22}

Organizations can benefit when they empower employees to speak up and advocate for certain features that they think are necessary.
\q{The philosophy at [redacted] is there's a significant amount of personal ownership over everything you do... We've realized now it's a little more effective to bring [decision making] closer to the source.}{P28}
It is unlikely that someone is an expert in all areas of the software and product, so organizations can utilize the collective wisdom from the team.   
\qs{I get to do those smaller sources of feedback and then using my contextual knowledge about how important I think this is, we can choose to fix it before it becomes a problem.... I [get my managers to] fight for this in the next meeting.}{P28}

In contrast, we observe some smaller or medium sized organizations having more traditional top down approaches to dealing with voices of users.
\qs{Yeah, the product owner would decide the prioritization of what the backlog looks like. And then in their sprint planning meetings, they would pull it into work to be done. I do not let the developers decide the priority.}{P14}
We found that founders or senior managers sometimes institute a separation of powers.
\qs{I think [once] the product team kind of has their vision as to what exactly it is that they need, then they'll start pulling the technical team because there's no point pulling us in any earlier than that until they know what they actually want.}{P15}

However, we observe that the organizations that foster individual empowerment, are the ones who benefit the most in terms of company goals and revenues \org{19, 21, 22, 31}.
Hence, there are clear benefits of empowering all employees when it comes to addressing the voices of users.
In particular, the empowerment and mobilisation of all employees provides more overall support to product management. 


\subsubsection{Active Feedback Collection}
The next crucial step in the process of becoming high performing is to employ the practices required for an organization to understand which sources are key to their product. 

To effectively gather and incorporate feedback from users, organizations should identify and utilize at minimum two sources that are representative of at least two of the ``voices of users" categories (social media, conventional feedback, and user usage metrics). 
To excel in this criteria of high performance, an organization must enforce the aforementioned technique of source consideration as a standard practice.
Organizations should also regularly review and update the source pool to ensure it reflects the changing needs of the organization and its customers.

In addition, as highlighted by many of our interviewees, companies can benefit from having a dedicated role or team to disseminate all the various user feedback sources.
Despite data scientists and data analysts roles becoming ubiquitous in software organizations, the volume of data is vast.
\qs{You have logs for everything. There's almost too much data. I think that one of the biggest issues is who's interpreting the data who's making the dashboard.}{P22}
This means that these organizations must allocate resources to not only collecting user feedback, but also interpreting the data. 

Some of the successful organizations reported having dedicated teams (marketing or public relations teams) to collect and manage the different sources. 
\qs{I think there are a couple teams that are dedicated to look into those. ... like what are the users talking about? What do they like? What do they don't like? ... I'm always getting those emails saying users really love this feature.}{P26}
Additionally, organizations may also benefit from roles that are cross cutting in nature and who understand the various sources of user feedback such as a customer support agent who has knowledge about user usage metrics in addition to conventional user feedback sources. 

As a whole, our interviews with the participants reinforced the importance of resource allocation within an organization in the form roles for successfully identifying the related sources. 
By utilizing multiple sources of feedback companies can gain valuable insights and understanding the needs and preferences of users which is essential for companies to become high-performing organizations.

\subsubsection{Active Triangulation} \label{sec: active triangulation}
Triangulation is one of the critical steps in managing the ``voice of users'' life cycle.
To be considered as high performing, an organization must triangulate their identified ``theme'' from a feedback source with at least one other source from a different category of ``voice of users''.
By following steps described in section \ref{sec: validation}, organizations can verify whether a specific user feedback has validity or not. 
For example, if an organization notices that users are complaining about the UI of the landing page on Discord and determines that it is an emerging theme. 
The organization could triangulate this theme with user usage metrics to gauge whether or not users are spending less time on the landing page or bouncing from the landing page. 
Triangulating the two categories of feedback in this example, social media source and user usage metrics, would significantly improve the validity of the theme.

Organizations perceived as high performing reported actively practicing validation before making any decisions about the feedback.
\qs{if someone says, this is a problem, we have a lot of data sources that we can then query to verify that that is a problem. And like, hopefully, if someone's DMing, you put in some amount of work to justify this as a priority.}{P22}
The process of triangulation would also require coordination amongst different roles and teams in the organizations. 
Data teams would communicate findings from user usage metrics with findings found from product, customer support, and customer success teams who are more closely in touch with conventional and social media sources. 
This aspect relates to the aforementioned factor in section \ref{sec: active employee participation} ``active employee participation" where \emph{every} employee is encouraged to be cognizant of the feedback and product.
This may open new collaborations and communication channels with cross-functional teams as different teams share responsibility in validating user concerns. 
\qs{I have to bug the [product people] often [for] validating because there are customers that are louder than others, you have to factor in that they could just be one very squeaky wheel. If one customer complains about it, there could be a myriad of customers behind the screen who haven't said anything about it, but it is a problem for them. So using data to validate.}{P12}
An organization can enforce better coordination and collaboration culture to maximize the effectiveness of the validation stage. 


\subsubsection{Active Response}
The final factor for an organization to become high performing relates to an organization's agility in responding to the ``voices of users."
Active response is implies responding to a feedback based as quickly as possible.
The response can be either a message or marketing post to the end users addressing the issues.
It could also correspond to fast development and release of the feature.
In both cases, the time of response varies depending on the complexity of the user feedback. 

Our participants explained it is not only sufficient to pay attention and consider important user feedback, but also respond to those feedback, particularly critical feedback, as soon as possible.
We know from previous literature that user feedback if left unresolved, can lead to cascading consequences that impact an organization's reputation and even bottom line \cite{li2022narratives}. 
Sometimes, this could mean that an organization shifts priority due to a sudden emerging user concern.
One participant highlights a notable example where responding to important user feedback and shifting priorities in a timely matter is paramount. 
\qs{I actually think a lot about the [redacted] security updates that occurred following some criticism [on social media] when [redacted] was really [popular].
[Redacted] very quickly shipped some very good community safety and encryption changes. And they shipped them so quickly that I [think] they were already being developed. It came down to a matter of prioritization and how much that they publicly showed what they did. Priority changed, and how its message to customers changed because it's quite a bit easier to change priority and messaging.}{P1}

This approach shares similarities to the principles of DevOps, which principles encourage an ``organization's ability to deliver applications and services at high velocity."\footnote{\url{https://aws.amazon.com/devops/what-is-devops/} }
In the case of DevOps, organizations are measured by their lead time for a change among other metrics to gauge an organization's ability to release code in small iterative batches. 
However, for active response, it does not necessarily always mean that an organization must ``release" new code right away.
An organization's response to user feedback could be in the form of a new version of software, but it could take form in its messaging or marketing.
As explained by P13, customers value the prompt response even if the product roll out takes time, 
\qs{What we found with [following up] on customers, they really appreciate that... I think, sometimes they paint these stories in their brain that like, I gotta reach out to [customer] support, [they're] going to take days to get back to me, there's going to be so much back and forth. And I think something our customers are always a bit surprised by is they're like, oh, wow, you actually follow up with with me, after you've released this fix.}{P13}



% Our interviewees further address the need for tools in a company to gather feedback and insights about products and services. 
% \qs{lots of ideas can come from the social media post. I don't know if this kind of tool is available in the market or not?}{P20}
% They also highlight that the absence of tooling in social media makes the process highly manual and time-consuming. 
% \qs{There's also no tooling that we have in social in order to actually catalog that count that, and it would be an incredibly manual process for someone to actually sit down and read everything and try to, you know, code it in a way that we could do something with it.}{P35}
% As a whole, our conversations with the participants reinforced the importance of resource allocation within an organization whether in the form roles or tooling for product management. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%Findings from V2






Notes: 

Our paper will provide a comprehensive overview investigating how software organizations conduct state of the practice analysis in using all forms of user feedback including social media. Combining that information with user metrics from tools like google analytics, hotjar etc to derive trends in user actions and concerns. 
Previous papers talk about user feedback and how it's important to consider them. In our study, we are looking into how social media can be a big part of voice of users. 
Although social media utilization doesn't seem like a big finding, we can argue that why are companies not using social media if it's that obvious. If it was so easy and straightforward then all companies should be using it. So our study will highlight why aren't they using it, what are the obstacles. 
We can provide a diagram/framework about the lifecycle of feedback. 


Flowchart of what's the state of the practice for how we should deal with voice of users. It comes internally, outside, social media, product managers. Once the information is acquired/taken it goes to the next steps, then gets deployed. After deployment someone has to look over the metrics. A new role is required whose job will be to oversee these usage data. What are people saying and doing. 
Data from voice of users are connected. All the data about the users, how they use the product, what they're saying about the product, it needs to come back to the feedback loop. This needs to be documented, recorded and further analyzed so better decisions can be made for the product in future. 

Concepts to talk about:
- Social media analysis: a form of user feedback. 
- Narrative angle: drawing from topic modeling. Topic modeling is done to gather idea about the topics that we see in the feedback. Similar to clustering. Finding the narrative behind these topics. 
Narratives impact user behavior. A narrative is something where you can trace a direct impact in usage metrics with something that you see in user discussion. For example: We see a pattern on Reddit for like maybe a button isn't working it broken and we see similar behavior change in hotjar like people can't click something because it's broken. 

DevOps and User feedback connection. Fast iteration. 
2023 update on s/w requirement. 

% \textbf{RQ1: } What practices organization adopt to manage trends in user feedback?
% \\
% \textbf{RQ2: } What challenges affect software organizations in managing trends in user feedback?



% \subsection{What are the different channels of user feedback used by software organizations? (RQ1)}
% \subsubsection{Conventional User Feedback}


% The triangulation process most likely requires coordination from multiple teams as data teams (i.e., data engineers, data analysts, etc.) must communicate findings from user usage metrics with findings found from conventional (i.e., product managers, customer support agents, customer success agents, sales, etc.) and social media sources (i.e., product managers, marketing, 
% and the introduction of tools and processes to support it, but the rewards are also evident. 
% It it beneficial for organizations to valid and learn which features and bugs are relevant and impactful for users before dedicating valuable engineering and product hours.

\subsection{What are the different channels of user feedback used by software organizations? (RQ1)}
When it comes to managing user feedback, the first critical aspect is identifying where and what to look at. This requires identifying the community of potential and current users of a software, product, or service. As noted by P3, a successful organization should collect feedback from \q{the community, [which] may consist of like-minded people working in the same space, who understand the industry's pain points and the ecosystem.}
Our participants described a variety of sources that capture user feedback from the \textit{community}, which include \textbf{\emph{emails, phones calls, video conferencing, product forums, support tickets, social media (e.g. Reddit, Twitter, Facebook, and YouTube), app reviews, user workshops, user interviews, surveys, and usage metrics}}.
Given this variety, we split these into three categories: inbound, outbound, and usage metrics and describe each of them in more details in following subsections. 

% \paragraph{Challenges}
% \q{It's really just trying, kind of firing on all cylinders, like, you know, using exhausting all the methods that we can be at a small change in our app, you know, running more email campaigns to solicit feedback through quick surveys and getting in touch that way. (P13)}

\subsubsection{Inbound Feedback}
One of the most significant and common types of user feedback is inbound feedback (NOWSHIN mentions). 
It may take the form of emails, phone calls, video conferencing, support tickets, and app reviews. 
\zane{nowshin list orgs for each example}
In these examples, users may directly request a response or a reply from a software organization through email, phone call, or support ticket where something in the software likely does not work and a customer support agent is directly needed to help the user. 
% As the most straightforward and easiest form of direct user communication, feedback from users via email, phone call, or chat support is used by all of our participants. 
\qs{We collect [user feedback] in all different forms. We do, you know, direct feedback from the customer via email, phone call, or chat support sort of thing. So that can come in through our CSMs, or through our tech support channels.}{P10}  

% Observing what competitors are doing is also a valuable source of feedback (NOWSHIN mentions). Several of our participants noted that keeping an eye on competitors' product road maps and activities is critical to understanding some of the important concerns of users. For example, \qs{join their open slack group and post questions there and view the helpful community questions in there}{P5} and similarly, \qs{and then other customers [sic] tell us something. You can get a sense of how your [products] are doing or how your competitors [products] are doing.}{P16}

 
Some organizations also choose to create their own community forums to gather feedback.
As P10 noted, \q{We also have an online community that our company built, it's kind of like open source feedback. We can go in, you can ask questions, and you can upvote different feature requests to see if you know, something would align with your business as well.} 
In theory, if enough users are active on the product forum, they would get a voice in influencing potential feature ideas and direction of the product. 
Other platforms, such as Slack, can also be used to collect user feedback collaboratively. For example, P9 noted that their company uses Slack to create shared channels for collaborative engagement with users, which sometimes feels like customers working alongside the company.
\qs{It's very collaborative, almost sometimes feels like, customer is working with us in the same company. [It] happens very organically through, [sic] threads and support tickets and retrospectives and stuff that we have after a major release.}{P9}

For software organizations that develop mobile applications, user reviews on Google Play Store and Apple App Store are crucial to the direction of product development (NOWSHIN mentions). P36 noted that at their scale, they receive thousands of app reviews a day and that several employees have dedicated roles to reading and analyzing app reviews. \qs{Four people that actually did that work. But we all did we all we all had access, and it was kind of our thing. It's like, we all got kind of into looking at the comments.}{P36} 
For these app developers, staying on top of major changes to the underlying operating system or phone version, is crucial for anticipating impacts on users. Even after testing a version of a new app release, people may still miss things during app testing, making it necessary to monitor the app release constantly.
\qs{We would always watch the app store when a big iOS release would go out, or a big Android release... we would all watch the feedback... people are human, and they miss [bugs]. So looking for [feedback, comments and] sentiment, drops or rises in star rating... it'll give you a pretty good feel for one of those two things, the new version of the app or new version of the operating system. [What] caused the app to not be driving the same level of sentiment.}{P36}
Though it should be noted that not sources of feedback is applicable for all organizations. 
App reviews would only make sense if an organization is releasing mobile apps and similarly, an organization can only unleash the benefits of a product forum if users are actively engaged in using the system. 
Overall, staying on top of user feedback is critical to developing successful products and services. Inbound feedback through phone calls, emails, product forums, and app reviews are just a few of the many ways that companies can gather feedback to guide product development and improve user satisfaction.

\subsubsection{Outbound Feedback}
Outbound feedback refers to the feedback that is actively sought by the software organization, rather than waiting for users to provide it on their own (NOWSHIN mentions). 
Our participants shared various methods for obtaining outbound feedback. For example, P9 mentioned, \q{One of the things that I did is went down to the lab in [redacted] in December and sat with the users and went through things with them. [I] took notes and gathered feedback. It is face to face [and] way more useful to look at it from that point of view like going into the lab as the users are using it and watching them play. We bring back all this feedback for the different teams that need to hear them.} 
This illustrates how face-to-face meetings with users can be a valuable source of feedback. 
Another way to receive outbound feedback talking to customers through technical support teams and assuaging concerned users, \qs{[our technical support teams] talk to customers and make make sure that if they're not getting what they want, perhaps we could at least soften the blow a little bit by by redirecting them to other things, you know, like other ways of on a customer service front to to sort of do that.}{P11}

Moreover, being proactive about getting user feedback involves setting up automated email communication, \qs{We have some automated email communications all teed up ready to go. That will basically detect if a user is using a certain [version], they'll get that sent [via] email... you've been using this new version for, let's say, a week, we want to know what you think.}{P13}
However, acquiring outbound user feedback is not only about offering the form feedback, but also providing time from the product manager, \qs{we're going to offer them the opportunity to fill out a quick survey, and also book in a time with me, they don't have to, but basically putting it in there like, Hey, do you want to book in a session with our product manager, and it's just connected basically directly to my calendar, and I'm hoping that people will look in with me and give me their feedback, you know, good or bad.}{P13}

Another strategy used by organizations, particularly large and resource heavy organizations, is the use of user workshops to collect user feedback (NOWSHIN mentions). 
In these instances, users are often brought into organizations and asked to test software products as organizations observe and analyze the users. 
\qs{We've got like a user research group. There are a team of people that would actually ask the public, the public obviously need to sign NDA, if they're exposed to some part of the game that's still on research. Then [we] basically record these sessions and watch how they do.}{P38}
An organization can also take advantage of a user research lab to conduct focus group session with users.
\qs{We have a we [a] user research lab... There's cameras in the ceiling [sic] cameras on the walls, and they can even even get these headsets you can put on that actually track your eye movement... The research team would hold these sessions and show [users] some products and let them play with it... They'd watch how they use the app. They would watch how they scrolled on the website. And they would record all of it.}{P37}
P37 further describes that the lab was very expensive, but it allowed the organization to study user interactions with the product in meticulous detail. 

In some instances, organizations would go out to the public, such as coffee houses and ask people to use their software products.
\qs{Sit in coffee houses and watch people. And we joke you're watching people doing coffees... but I'm watching how they communicate, how they use their devices... sometimes talking to [users and asking] you're doing this thing with your phone and [how would you do this and why]}{P37}
Similarly, \qs{We would go to coffee shops. We'd sit there maybe with a computer and [something] to show about our [website] or maybe our [app]. And just talk to users and say, ``Hey, we're thinking about doing something that does blah", and just literally just have a conversation with users about, oh, this is a cool idea. ``Here's what I think you should do. I saw this somewhere, maybe be cool." If you do that, and just talking with them, coming up with some ideas, doing some ideation on [sic] maybe what some features might look like.}{P36}
The central benefit of the user workshops is that they facilitate observations and analysis of users utilizing a software product in front of the organizations. Organizations get a full in-depth view on how and why users are utilizing the product. 
The consequences are also ostensible. Conducting these user workshops whether in the form of focus groups and interviews is time intensive and require specific research roles that are not accessible for any organization. 

Outbound feedback can be obtained through a variety of methods, including face-to-face meetings, surveys, interviews and user workshops. 
These sources can complement inbound sources to help organizations proactively gather feedback from their users and use it to improve their products and services.


\subsubsection{User Metric}
When it comes to user feedback, user metrics from software usage can provide valuable insights for software organizations (NOWSHIN mentions). 
Organizations are incentivized to collect these metrics as \qs{the metrics don't lie. Metrics [have] no face... they're just raw data. And you can look at that raw data in lots of different ways. Sometimes it's about how a new feature or change you made, sometimes it's about a bug, [sic] you always look for what's the cause and effect of a change in a metric.}{P36}
Almost all of our participants collect some form of usage metrics as users use a software product. 
Given the cost of conducting interviews or user workshops, usage metrics offers a more accessible and cheaper solution for organizations to record how users are regularly using their product. 
We found that our participants from smaller organizations are frequently at the forefront of adopting tools for collecting metrics. 
P6 describes how their organization can visualize user behavior, \q{where they clicked [sic] Someone tried to use search feature. [sic] User did a lot of events with us. Seems like it's a repeated user. They saw the menu. They did a lot of click events. They clicked on the restaurant title name for some reason.}
Similarly, P2 uses tooling to record, \q{how many people stay and how many actions are doing you can play, what they are doing on your platform. So where the mouse is going, where they are looking at how much time they spend on a specific feature. And that's going to help you understand how people are using a product. So it's it really shows you what people are doing.}

We also observed medium sized organizations heavily relying on user usage metrics to gain insights on user behavior and triangulate with inbound and outbound user feedback.
\q{There's always going to be people who encounter issues, but don't reach out. Customer usage data from what we gather on our back end [paired with] continuous communication with a support team to advise us on what they're seeing, and what what is most popular}{P13}
P10 also describe their organization's usage of tools for analyzing feature usage, \qs{
Pendo is kind of cool. Because it tracks every click, [sic] you can go into it on a user level and see exactly where someone clicked, at what time, and they generate these fantastic graphs for you that say, you know, this person spent 80\% of their time on this one.} 
Large organizations also take advantage of collecting usage metrics as P35 explains \q{And imagine tracking what users are actually typing into that search bar, and then tracking what successfully resolves to, you know, to where they successfully get to what they needed versus where we couldn't fulfill their search requests.}

Overall, tracking user metrics is an essential part of managing user feedback. It allows software organizations to gain valuable insights into user behavior that the organization can leverage to triangulate with the qualitative data gained from the inbound and outbound feedback which can be used to make informed decisions about product development and improvements.

\subsubsection{Challenges}
Collecting user feedback can be a challenging process for software organizations.
According to P6, one of the biggest challenges is a lack of engagement from users to provide user feedback (NOWSHIN mentions).
\qs{We have feedback mechanisms in place, but no one seems to be using it like no one is filling out our feedback forms, [sic] giving star ratings or nothing... I know it comes with some reward benefits.}{P6}
In particular, smaller organizations face an extra hurdle as they may not have reached critical mass in the number of users to receive consistent amounts of user feedback. 
As some smaller organizations are undergoing transformation and growth, they are amidst great adjustments, \qs{Because of that services organization mentality, most of the feedback happens with things like [sic] post mortems.}{P9}
Sometimes, the nature of the software requires users to come to the organization's office for the organization to collect feedback, but this may not be possible in reality. 
\qs{We [develop] this [feature] over the year. To get user feedback... you cannot ask a [user] to come out to your office. But you need to figure this out anyway.}{P34}

Another challenge is obtaining feedback from users who may dislike the software and have genuine reasons why they do not want to continue using it.
\qs{Usually you won't get good user feedback from people that dislike your product. [sic] So if someone that's turning from your product, and you're trying to do an exit survey, like why did you leave, what are we missing, they're not going to spend that time, unless they're incentivized.}{P14}
One tricky trade-off that organizations must balance is obtaining the adequate consent from users to collect feedback, \qs{One of the challenges is [sic] consent. [We] had a very limited [number] who they can reach out to, and let's say out of 100\%, just 30\% consented for that and out of 30\%, [4 or 5\%] maximum responded to the service.}{P31} 

Collecting user feedback can be a challenging process, but our participants highlight the importance of collecting feedback from users, best explained by \q{it is very, very important to be talking to your users to be talking to your customers. Otherwise, you're going to build what you want. And you're going to miss probably 99.9\% of what everybody else wants.}



\subsection{How do software organizations leverage user feedback from social media? (RQ2)}
\subsubsection{Monitoring Social Media}
In today's digital age, social media plays an important role as a public square for user discourse about software products. 
Social media has emerged as a crucial tool for organizations to connect with their users and gather valuable insights about their needs and preferences, representing a new and powerful outbound feedback gathering source. 

% A key aspect still imperative throughout the validation step is that it is important to focus on trends and themes rather than individual comments. 
% It is simply not feasible to respond to every single piece of feedback, so organizations need to look for patterns that indicate broader issues. 
% One effective way of doing this is by taking a random sample of users or targeting those who are highly engaged with the product or service.
% \qs{You don't need to look at every single [comment] because a trend occurred. You just take a random sample of the users, and sample based on some level of engagement that makes it a bit more useful.}{P1}

Our participants discussed how their organizations monitor a variety of popular social media platforms including Twitter \org{1, 2, 5, 11, 13, 17, 18, 22, 24, 25, 29, 30}, Reddit \org{1, 2, 12, 16, 17, 19, 21, 22, 25, 30 }, LinkedIn \org{7, 12, 21, 23, 29}, Facebook \org{17, 19, 27, 31}, Instagram \org{1, 17, 20, 31}, Discord \org{1, 2, 5}, YouTube \org{1, 23, 30}, and TikTok \org{17, 25}.
From Reddit to TikTok, proactive organizations are constantly monitoring their online presence to determine what people are saying about them. 
These conversations reveal the potential bugs and features that may impact these organizations, big and small, in various industries.

For example, in one interview, a participant revealed how at their organization, they have a dedicated team who monitors social media feedback on Reddit. 
\qs{There is a good amount of social media involvement in the [sic] Reddit posts... Not only PMs, I think there are a couple teams that are dedicated to look into those. Always. They always check and we get monthly emails what are the users talking about? What do they like? What do they don't like? Like, I know that there is a [product] feature that users really love, they're always talking about it that they love that.}{P26}
This feedback helps the team identify issues and features that users like or dislike, and monthly emails are sent out to report the findings. 
In essence, the trends that emerge from large volumes of feedback on social media serves as a useful part of product and engineering teams.
\qs{We have a team that just looks at social media, and they report on like, the biggest \textbf{trends} coming from social media. I mean, because you can imagine this company is in the news all the time. So yeah, we it's definitely a part a part of our weekly life of what we look at.}{P27}

Similarly, an interviewee from the gaming industry revealed how social media monitoring is essential for live games. 
P32 explains how their organization utilizes Twitter and other social platforms to receive real time updates on user concerns and reporting on bugs.
\qs{People tweet. So there are different channels they [talk]... Our [product managers], they monitor those channels. Because [redacted] is a live game, if something is impacting the people, [they] complain in those channels. And we see that.}{P32}
The organization's product managers monitor various channels to identify issues that impact users and quickly engage engineering teams to address them. 


We found something that is unique to the gaming industry is the impact that ``game reviewers" have in driving a trend that goes viral on social media.
These trends could snowball and force these software organizations to respond.
\qs{We look at a lot of different sources... Twitter... Reddit is another common one... \textbf{One YouTuber} [highlighted this]. In [redacted], there are these things [features that] players could pick. For this year, the game team decided to revise how the system works?...So there were a lot of negative feedback from the community through public channels talking about [it].}{P38}
Social media feedback is just one of the many channels used to ensure that the game runs smoothly and meets user expectations.

Moreover, social media monitoring is not limited to just one platform. 
For some organizations, they just monitoring sources like Reddit and Twitter is not enough, they have to also listen to inputs from big trade shows like CES to help gain a holistic view of their industry and make data-driven decisions.
\qs{Anything about [our product], so there's a pretty strong social media strategy that's there. And it's not just what do we put out, but I know I'm sure it's also what comes in, and then have the inputs then get distributed, just like any other inputs from listening sessions or from any of the big trade shows [like] CES}{P37}

To gain insights from their respective ``communities", our interview participants went to great lengths to uncover feedback from social media.
\qs{I'm asking questions [on Discord]. And generally I don't ask question under my name. I have some fake names that I use... So I have some fake name with a male and a female account question because [sic] you need to [reduce] bias. Some guys want to seduce a girl and some guys are gonna be aggressive with [me]. So I'm basically trying to have neutral data points non biased, you always going to have bias, but your goal is to reduce bias.}{P2}
To mitigate against potential biases that users may express in online social media, this participant not only uses pseudonyms, but also converse with their community via female and male profiles.

However, social media monitoring is not just about gathering feedback. It is also about identifying trends and staying ahead of the competition. 
\qs{One of our competitors, [they're] on LinkedIn. And [they] just leak information all the time. [They] posted a link to their internal feature requests... I was like, ``Oh, thank you very much. I'm gonna take a look at all the information you have here. And we're gonna pull it down from this, because it's public."... So now I can turn around and have our marketing team create a marketing push.}{P14}
Companies have to be able to react quickly to changes in the market and adapt their strategies accordingly. This means monitoring not just their own brand, but also their competitors.

Social media monitoring is a crucial tool for businesses of all sizes and across various industries. It provides real-time feedback from consumers, helps identify trends, and allows companies to quickly address issues and improve their products. 

\subsubsection{Challenges and Limitations of Social Media}
While our participants immersed us with examples of their collection of feedback from social media, they also listed some challenges associated with feedback from social media that need to be addressed.

One of the challenges is that not all the organizations can benefit from social media. While all the consumer facing organizations can benefit greatly from feedback from social media, it may not be as useful for organizations that have fewer, but bigger customers. 
\qs{There is [not much] social media use cases. In our Facebook, [we get] only 1000 like so.}{P40}
This can be a limiting factor for any organization where they are building bespoke software and have a handful of users.

When feedback from social media is collected, the quality of feedback from users should be scrutinized.
Social media feedback can often be vague and lacking in detail, making it difficult for organizations to get an accurate picture of a problem or feature. 
\qs{The problem is the quality of the feedback from from customers. It is very different from when a customer would reach out and fill out a form of support form. Those types of tickets are more reliable type of feedback compared to social media. Social media, they're often vague... ``It's not working at this account," but, "What is not working?"... There's a lot of details that are missing from that [social media] interaction.}{P11}
This is why an organization may need to reach out to users and ask them to fill out additional surveys and/or interviews to gather more information.
\qs{So you'll notice that some companies would then reach out to the customer and say, ``I can [help] you, thank you for reaching out, can you fill up a form so that we know you're real and you can give us more detail about the problem so that we can solve it?"}{P11}

Another challenge associated with user feedback from social media is the amplification factor. 
Pure volume-based analysis may be misleading, as social media can amplify certain features or conversations, regardless of whether they are valid signals or not. This can lead to misinterpretation of trends, and companies need to be aware of this when analyzing social media data.
As explained by P1, \q{I think that a lot of times, when you're doing just pure volume based analysis, you run into that problem, because social media has a huge amplification factor that you have to be aware of. If someone starts talking of a particular feature, more people will start talking about that feature, or more people will start talking about a particular thing.}

Related to the amplification factor is the potential for noise that organizations can collect as part of the feedback.
Sometimes you see a bunch of complaints, but these complaints are not directed at the software product and instead some unrelated aspects.
\qs{Facebook was [used]. And I would say, people used to complain a lot. I mean, like, whenever people, things work fine. People don't compliment in [Facebook]. But the thing is [the] majority of complaint was actually unrelated to us. Because most of the time, it was complaining about [something unrelated].}{P34}

From social media, some interviewees expressed that bugs are widely reported, but feedback regarding on feature requests are more scarce overall.
\qs{We noticed we only got negative feedback through social media or like positive reviews. It was never [sic] feature requests. It was mainly [sic] someone's having an issue with a bug, or they just really liked the product}{P17}

Based on our interviews, we found that many small, medium, and large organizations use social media feedback in some capacity. 
One of key limiting factors to more widespread adoption is that it is currently quite ad-hoc, with no formal way.
Even in large organizations where they may attach dedicated teams to collect social media user feedback, this is conducted through manual means.
\qs{There's also no tooling that we have [for] social [media]. [Nothing] we [have] to actually catalog [and] count that. An incredibly manual process for someone to actually sit down and read everything and try to [sic] code it in a way that we could do something with it.}{P35}

Despite the aforementioned challenges, ultimately, a lot of users will choose to join and leave a software product depending on perception of the product and trends on social media.
As explained by P24, \q{A lot of business will come from reputation. Whether people recommend and stuff offhand. ``Oh, you should use this, or this is really useful for this sort of thing." So social media can either enhance or damage your reputation, and that will directly affect the business in many cases}.





\subsection{How do software organizations manage user feedback? (RQ2)}

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.95\linewidth]{figures/VoiceofUsers.pdf}
  \caption{The Generalized Data Flow of the Voices of Users. \\ (A) represents the data flow of the ``Voices of Users". (B) represents the life cycle of user feedback as part of software development process. (C) indicates the 3 categories of user feedback that formulate ``Voices of Users". (D) indicates the transformation of user feedback throughout different stages of the user feedback life cycle.}

  \label{voice-of-users-data-flow}
\end{figure}

Once an organization identifies and collects a stream of user feedback from a variety of sources, the next fundamental step is managing this trove of feedback.
Our interviewees come from diverse software industries and organizational sizes, but they share commonalities across the management and usage of user feedback. 
For an organization that strives to understand its user requirements, perception, and areas for improvement, it should adopt methods to listen to the \emph{``Voice of the Users"} as well as effectively managing it. 
We captured these commonalities and present them in a generalized data flow 
of the \emph{``Voice of the Users"} in Figure \ref{voice-of-users-data-flow}.
In the following subsections, we describe in details the main steps in managing user feedback 1) analysis, 2) validation, and 3) prioritization.
\nowshin{Should add a definition for voice of users?}

\subsubsection{Analyzing User Feedback}
Analyzing user feedback is an essential part of understanding user concerns and requirements to develop successful products and services. 
It allows product managers, developers, and senior managers alike to gain a deeper understanding of user needs, preferences, and pain points, enabling them to make informed decisions about product features and bug fixes.

The main purpose of the analysis of user feedback is to find emergent trends and common themes that develop from the user voices. 
Part of the process is listening to the bastion of user voices and group similar patterns.
\qs{What are the things that they struggle with. [We] went through all that feedback and grouped the similar themes about what were the common complaints and and what were the common dream features that everybody wanted.}{P4}
The same question repeated again and again is often representative of a underlying problem. \qs{The number of times the question was raised was also important, because that means many, many [users] are having this confusion.}{P5}

Our interviewees all shared with us the importance and main goals of finding the ``themes" in the feedback.
\qs{Ultimately, it's about the themes. It's looking for other patterns in the comments... We released a new version that was 100\% deployed in the App Store. All of a sudden, we're starting to get some some tanky reviews and people complaining that [redacted] are slow. Because you know, you're always looking for something to appeal to, to the large majority of people.}{P36}
When customer complains through support channels, the volume of complaints can illustrate trends as well as explained by P14, 
\q{You got a trending amount [of] support tickets complaining about a specific issue.}
An organization cannot expect to satisfy every possible user out there, so identifying the common themes will help uncover the potential bugs and features that matter for the masses.


However, analyzing user feedback is not a straightforward task, and there are several important considerations that must be taken into account.
One key point that emerged from our interviews is the importance of balancing high-level feedback with detailed feedback. 
As P27 noted, if an organization wants to dive deep into an area, then one-on-one interviews or sessions with small groups of users are necessary. 
This type of feedback allows product teams to gain a detailed understanding of how users are interacting with a particular feature and whether it is providing the intended value. 
In contrast, P27 notes that high-level feedback in the form of NPS or thumbs-up/thumbs-down ratings can provide a quick and easy summary of overall success. 
Both types of feedback are necessary for organizations to make informed decisions and push a product forward.

When an organization takes the advantage of social media user feedback, it can provide rapid insights on bugs the occur.
\qs{During the testing process. We missed [including the menu items]. We woke up one day... All these messages on social media being, ``what the heck, I just updated and none of the menu items [exist] anymore." }{P13}
We see the importance of pure volume of feedback manifesting as a key factor of identifying themes.
% \qs{People will post snapshots of a Reddit post with a whole bunch of votes. And [users are]  mad about the seat heater, or on the new UI. And then a month later, there's a JIRA ticket and someone's working on it. So}{P22}
For organizations that dedicate the resources to monitor social media, our interviewees explained the importance of paying attentive attention.
\qs{On Twitter [and] LinkedIn, there's a ton of different accounts that are out there. [We] monitor those. And I also know that anything that I say on social media that has anything to do with [our product with] a hashtag, they [will] pay attention to that. We [also have] Instagram and [are] aware of people send their feedbacks and based on that [our] team [will] decide whether to develop the feature or not.}{P38}

However, P38 also points out that it's essential to balance the signal-to-noise ratio and consider which groups of users are over-represented or under-represented in this type of feedback. 
After all, some groups may be more likely to post on social media than others, which can skew the data. 
It's important to ensure that the feedback received represents a diverse range of users and is not biased towards any particular group.
Identifying themes can also be tricky and onerous, as P18 explained there is a lot of manual reading of user comments and organizations may not actually understand what users are saying.
Based on conversations with our interviewees, disseminating themes from user feedback is still an overwhelmingly manual and laborious process.

Furthermore, analyzing user feedback requires an understanding of the limitations of the data. 
Users may have conflicting opinions or report pain in the spur of the moment.
\qs{A lot of the time, requests come in, they're not flushed out fully. In the moment, they're frustrated with something. And then two hours later, [they] don't need that}{P14}
It is crucial to listen to all feedback, but it is equally important to recognize that not all feedback is equal.
From analyzing user feedback into themes, organizations can gain a deeper understanding of their users and pick out themes that represent important features and bug fixes for future product iterations.

\subsubsection{Validating User Feedback}
The next step after analyzing user feedback and identifying themes is validating those themes that emerge. 
In particular, how does an organization know that a specific user feedback is valid or worthy of action?

The potential consequences of misinterpreting themes are significant. 
\qs{The movie Morbius became a meme... The core of the meme was that no one had actually seen this movie. [Discussion] became very popular. Sony actually extended the theatrical release of the movie, because they saw a trend that the popularity of the movie was increasing. They did not test to determine that the reason why the popularity of the movie had increased is because people were having fun talking about how no one had seen or any intention of seeing the movie.}{P1} 
The end result was that the company wasted the money re-releasing and re-marketing the movie to no audiences \cite{mendelson_box_morbius}. 
Misinterpretation is particularly pronounced for user feedback on bug reports. 
A reported bug may be in reality a misunderstanding.
\qs{You first got to validate whether it is actually a bug or if it's intended design, sometimes customers will misunderstand the system. They'll file bugs against things that are designed as intended.}{P24}


The lifeblood of validating user feedback involves triangulation between all the sources of user feedback to reduce misinterpretations. 
26 out of the 32 organizations studied collect at least some form of user metrics which it critical to the triangulation of user feedback themes.
One can compare the themes from with conventional and social media sources with user usage metrics and vice versa. 
% Analytics are key to understanding user behavior and identifying potential areas for improvement. 
By tracking user engagement with different tooling such as Hotjar or Google Analytics, we can see which features are being used effectively and which ones are being ignored. 
These tools are sophisticated enough so that anyone at the software organization could replay a user usage session like a movie and visualize every button click, mouse hover, and delay on page. 
\qs{Everything is tracked, every click is [tracked], every action is tracked. That user feedback is how users interact with the [product].}{P39}

However, analytics can only take us so far, and organizations need to supplement this data with direct feedback from users.
\qs{We check analytics to see like who's using what, and then if someone's not using it follow up with customers and do a review.}{P7}
Similarly, 
\qs{Every big system has monitoring. So we will align that [with other sources]. [We see] people are complaining that they cannot log in and we will see in our graphs and charts. ``Oh, yes, the services down."}{P32}
The triangulation process most typically would require coordination from multiple teams as data teams must communicate findings from user usage metrics with findings found from product, customer support, and customer success teams who are more closely in touch with conventional and social media sources.
Establishing tools and processes to support this triangulation would require efforts, but the rewards for an organization is that has greater likelihood to verify which features and bugs are relevant and impactful for users before dedicating valuable engineering and product hours.

Triangulating user feedback may open new collaborations and communication channels with cross-functional teams as different teams share responsibility to validating user concerns. 
\qs{I have to bug [product people] often [for] validating because there are customers that are louder than others, you have to factor in that they could just be one very squeaky wheel. If one customer complains about it, there could be a myriad of customers behind the screen who haven't said anything about it, but it is a problem for them. So using data to validate.}{P12}
One possible strategy is starting with social media to identify themes and then directly contacting users to validate. 
\qs{Social media is a good place to get started. You find a trend. Next step is to collect a statistically relevant, smaller sample of genuine accounts that you care about.}{P1}

Validating user feedback is an important process with the end goal of using triangulation to mitigate misinterpretation and misunderstandings.
After this process, an organization would have collated a list of feature and bug concepts that were validated and represent genuine issues. 


\subsubsection{Prioritizing User Feedback}
In the next step of the generalized data flow of the voices of users, an organization should prioritize these features and bugs. 
Prioritizing features and bugs involves making trade-offs to ensure the organization gains the maximum benefit, particularly since small and medium-sized organizations often have limited development resources available.
Striking the perfect balance between trade-offs and identifying the most paramount feature and bugs is essential. 

As per our interviewees, the critical factor to prioritization is whether features and bugs match a company's vision and goals. 
Best described by P27, \q{if we get feedback, that doesn't align to anything we're doing.. [if] it's not something that we're going to address this year, we're not going to redesign it, we're not going to revamp it.}
That is not to say that they would completely ignore it, \qs{I'd probably look at little quick fixes I could make [it].}{P7}
The central tenet to an organization is revenue and profit so it is incentived to deliver new features and fix bugs that maximize benefit for the most customers. 
\qs{At the end of the day, we need to make money. If there is a feature that one customer wants and [has] a significant impact on revenue, we're going to implement the feature. [The] features need to be reasonable. If they ask to put a pink elephant on the homepage, we're not gonna do that. But if they implement a feature that's gonna benefit [many] people. Yes. We're gonna do that. But it needs to drive revenue.}{P2} 

The key to prioritization is balancing trade-offs so that there is mutual benefit for the users and organization. 
P6 astutely observes, ``if they [users] are giving us [feedback], it's likely...that [something] would help them. [They] help us because they are going to use our system."
However, not all feedback is created equal and the often ad-hoc process of prioritizing can result in the wrong decisions, which is particularly troublesome for smaller organizations with limited resources. 
\qs{Sometimes we end up choosing such a [feedback] to implement, which probably just takes a lot of time and we have limited manpower. [Alternative] task which [ended up] more important gets delayed. So we do make mistakes, but we try to avoid that by discussing and analyzing [if feature is] gonna contribute.}{P6}
Using one judgement to determine priority is echoed by P22, \q{it's just a matter of using your judgment, your best judgment is enough to determine priority... Have a clear discussion with your team and [say] this is important because XYZ and I'm gonna work on it now.}

Furthermore, the underlying driving force for major features is often the revenue that a prospective feature may bring to the organization.
As P23 discussed, \q{based on their requirement, we sit down with them and ask them some questions, what is the requirement, how important it is and how it can benefit our team and our company in terms of \textbf{revenue} as well... If the feature costs more than what they were expecting, then probably they will drop off the feature... is all based on budget.}
There may be limitations in terms of budget or resources and this shows that even if the feedback is important, it may not always be possible to act upon it immediately.

The company always prioritizes things that make money and prevent them from losing money. 
Of course, there are also practical considerations to take into account. 
\qs{In the current economic condition, the company always is prioritizing things that make us money and prevent us from losing money...[But] there's significant delay between feedback and effect... [May] take a month or two to really show.}{P28}
This means that even if feedback is prioritized, it may take time to see the results, but an organization can \qs{find small issues quickly and fix them.}{P28}
Such approach was corroborated by P30 who explained if it is a small feature request, it may be decided at the team management level. 
However, if it's a massive feature request, it will likely need to be approved by C level executives or other senior executives. 

However, it is not just about the financial impact. 
As another participant pointed out, \qs{people's perception of the company as a whole}{P28} is also an important factor. 
If the feedback is related to something that is damaging the company's reputation, it will be given priority even if it doesn't have a direct financial impact. 
After all, a company's reputation is invaluable and can influence user behavior to adopt or drop a software product. \zane{Cite narratives paper? LOL}
\nowshin{YES}

Another factor that emerged from our interviews is the trade-offs made between bug fixes and features. 
Different levels of priority are assigned to bugs and features based on their criticality and the team's assessment of customer impact.
One assessment strategy from P31's experience is creating Jira tickets with points allocated, and the intensity is calculated based on customer-facing teams' feedback.
New features often have to be scheduled into sprints and bug fixes usually take priority.
\qs{New features are typically lower priority than bug fixes. So usually bug fixes are prioritized top of the list, because it's something that the users are paying for or having issues with as compared to something that just doesn't exist.}{P17}
% This approach was also repeated by P15, who said \q{Typically maintaining existing revenue is very important. Whereas delaying new revenue is less costly.}

% Maybe drop this paragraph to save space
Organizations that provide software as a service (SaaS) are often bound by service level agreements (SLA) that stipulate penalties for unavailibility or other major bugs. 
We found that they too also prioritize bugs and other problems over new feature offerings, as P24 explained how features are lower priority because they guarantee that things won't be running properly. 
However, not all bugs receive this priority, as P25 conveyed, ``Even bug bugs also get like priority labels on them." This priority is dependent on number of affected and affect on revenue, but high priority bugs get fixed immediately, where as small bugs may linger for a long time.

Prioritizing user feedback is a necessary step that requires balancing trade-offs for features and bugs.
By striking this balance, an organization may create software that not only meet user needs but also align with their larger vision and goals.

\subsubsection{Development and Release}
At this point, an organization should have identified initial themes based on user feedback, developed feature or bug concepts based on the user feedback through validation, and prioritized the important features or bugs.
The last step of the data flow of the voices of users is the development and eventual release of new features or bug fixes from an organization's prioritized list.
This is the point in the data flow process, where the technical team is given the most responsibility to take the prospective feature or bug fix and develop the software to match user requests. 
When an organization finishes development and the new version of the software passes all the assigned tests, the organization will release the software to its users at the next opportune time.
Depending on the organization, this interval could range from minutes to months. 
However, when that new software version is released to users, a new cycle of the data flow of ``voices of users'' is triggered and new user feedback, good or bad, will makes its way to product managers, developers, customer support staff, data scientists alike. 



\subsection{How does ``voices of users'' fit into product management? (RQ3)}
In addition to understanding data flow for the voices of users, our interviewees helped share insights on the relationship between use of voices of users in requirements engineering and product management practices. 
From our interviews with participants, we identified three main points that organizations should consider for product management. 

\noindent\textbf{Individual Empowerment:} The first point we found is that large organizations \org{O19, O21, O22, O27, O31} often heavily encourage their employees to take the initiative, particularly for identifying issues in the software products.
% The placement of responsibility on developers and other roles involves identifying features or bugs in their daily work or even from social media outside of work hours. 
\qs{There's a lot of ownership among devs. If you're working on something, it's expected that you own that and see the potential risks and impact of you're doing and make design decisions for that.}{P22}

% Since employees have a stake and voice in the product, they frequently will pick out themes from user complaints on social media as employees are doing their regular browsing, 
Employees who are invested in the product may pick out themes in user complaints on social media while browsing,
\qs{High majority of [redacted] employees are also very interested in [redacted]. It's very common that the employees will frequent [redacted]'s subreddits. [Some] bug reports and feedback comes from internal employees being on [redacted] related social media.}{P22}
Therefore, employees frequently will post screenshots from social media regarding popular concerns that impact the product {[We see] screenshots of a Facebook post saying ``what does this alert mean?" And then someone's on it, trying to make the customer facing UI more understandable or adding something to the user manual. This \textbf{initiative} is definitely led by employees that have other jobs that just happen to be also invested in these kinds of things.} 
% P28 corroborates this sentiment, \q{The philosophy at [redacted] is there's a significant amount of personal ownership over everything you do... We've realized now it's a little more effective to bring [decision making] closer to the source}

In contrast, we observe some smaller or medium sized organizations having more traditional top down approaches to dealing with voices of users.
\qs{Yeah, the product owner would decide the prioritization of what the backlog looks like. And then in their sprint planning meetings, they would pull it into work to be done. I do not let the developers decide the priority.}{P14}
We found that founders or senior managers sometimes institute a separation of powers.
\qs{I think [once] the product team kind of has their vision as to what exactly it is that they need, then they'll start pulling the technical team because there's no point pulling us in any earlier than that until they know what they actually want.}{P15}
However, we see the benefits of individual empowerment when it comes to addressing the voices of users.
In particular, the empowerment and mobilisation of all employees provides more overall support to product management. 

% Placement of ownership on employees does not come without negatives as employees end up with more work overall.
% \qs{The cons is that you end up working way more, because you're basically you're doing like multiple jobs.}{P22}


\noindent\textbf{Impact on Requirements Engineering due to Discrepancies with DevOps}
From conversations with our participants, we found a discrepancy between the theorized rapid iterations and quick feedback loops championed by DevOps and continuous integration \zane{cite} with what organizations practice in reality.
For some of our participants, we found that they often planned their product road maps 6 months or even 2 years in advance. 
This process is of planning the road map is not entirely based on user feedback, but also relies on company goals and visions.
Despite the whole concept DevOps which facilitates quick feedback loops so that an organization can respond swiftly to market changes and changing user requirements, such long road maps may limit the ability to rapidly pivot.
For example, senior management may decide that they want to make a major change to the entire underlying software infrastructure, \qs{One big project is gonna kick off from next month, migrating everything to Google Cloud Platform. [Goal] of the company is to help improve user experience. The project is around 2.5 years worth of work. So for this entire 2.5 years of you know, duration the efforts and the points for the JIRA tickets are already set.}{P19}
Feedback may flow into the organization, but they cannot react to it in time.

When hours are already allocated it could limit what development teams are available to deliver based on new assignments that product teams assign. 
\qs{One of the biggest things that happens is timeline and feasibility in the time. Sometimes, [product] want this and the engineering team is like, we can't have that ready for in two months, but we can have ready in two months is this. And then another four months, we could have the full thing. 
So is there a way of breaking it down into like, more feasible deliverable chunks oftentimes are what's what are the intermediate deliverables that can be achieved in order to have something successful without it being like, too long in between things?}{P15}
Understanding the limitation that development timelines could have, an organization can still leverage user feedback to its advantage. 
\qs{I actually think a lot about the [redacted] security updates that occurred following some criticism [on social media] when [redacted] was really [popular].
[Redacted] very quickly shipped some very good community safety and encryption changes. And they shipped them so quickly that I [think] they were already being developed. It came down to a matter of prioritization and how much that they publicly showed what they did. Priority changed, and how its message to customers changed because it's quite a bit easier to change priority and messaging.}{P1}
Paying careful attention to user feedback can enable an organization to identify major fires and shift priorities.
The example also demonstrates why it is critical to manage user feedback, specifically social media, to curate a positive perception and messaging when software priorities change. 


\section{Discussion}
% \qs{I actually think a lot about the [redacted] security updates that occurred following some criticism [on social media] when [redacted] was really [popular].
% [Redacted] very quickly shipped some very good community safety and encryption changes. And they shipped them so quickly that I [think] they were already being developed. It came down to a matter of prioritization and how much that they publicly showed what they did. Priority changed, and how its message to customers changed because it's quite a bit easier to change priority and messaging.}{P1}
% Paying careful attention to user feedback can enable an organization to identify major fires and shift priorities.
% The example also demonstrates why it is critical to manage user feedback, specifically social media, to curate a positive perception and messaging when software priorities change. 

% Yeah, yeah. And especially, you know, startups, because the real struggle is, we don't know, the best practices out there. I mean, sometimes the things could be really easy. And there is already an established, you know, guideline to do things, but we just, you know, we explore and do and probably, you know, ultimately reach to the same point, what's supposed to be done. So after spending a lot of time. P6


\subsection{``Voices of Users": All data is relevant}
Summarizing all the findings here??? Maybe
% \subsection{Proposal for an Viable User Feedback Pipeline}
% We are proposing the pipeline. Speculate on improvement.


\subsubsection{Identify the low hanging fruits.}
Organizations utilize a wide variety of sources for user feedback.



\subsection{Identifying trends and its impact on user behaviour}
cite ourselves



\subsection{Social Media: The New Frontier for Product Innovation}
WHY Social media is important
use the Reddit example
there are tools out there, but industry does not use it very much
Social media a large scale 
As social media continues to grow and evolve, companies that ignore its impact on their business do so at their peril.

==> olderVersion.tex <==
Related work:
%Studies have tried to better characterize sources of user feedback with the term ``voices of users" \cite{tizard2020voice}, which tries to contextualize all the sources of user feedback.


% Understanding how organizations manage client-feedback and which challenges they face is important to organization sustainability. 
% According to Parida \emph{et al.}, sustainability encapsulates the management of responsible production such that corporate relationships and social environments are well preserved despite changing demands on a company's abilities \cite{parida2019and}. 
% Thus, to preserve organization sustainability it is essential that companies consider and understand potentials of user feedback, particularly given the constantly evolving nature of the various sources of feedback.


% This means that analyzing the voices of users requires more complex, intricate processes. 




% The analysis of user feedback is increasingly important for organizations to consider for product usability but also to maintain competitiveness in the market. 
% While traditional elicitation methods are effective to a certain extent \cite{van2021role}, listening to the voices of users helps organizations reap the benefits of feedback \cite{van2021role}.
% \hghlt{These methods may not take into account the evolving needs and preferences of users, as they often involve a one-time or infrequent gathering of requirements.
% }
% Traditional elicitation methods like surveys often rely on a small set of stakeholders or experts to define and prioritize requirements.
% While traditional elicitation methods like surveys, interviews are needed, they fail to capture the full range of user needs and perspectives \cite{tizard2022voice}.  
% Gathering voices of users can assist software organizations to increase their marketability, thus improving the success of the product as user satisfaction is increased. 










% \hghlt{
% These sources of feedback provide software organizations with unprecedented opportunities to obtain insights on issues and concerns.
%For instance, organizations can manage these sources to identify potential important areas of improvement such as new features or bugs to repair.
% However, a comprehensive understanding on how organizations manage user feedback to improve existing products is quite scarce. 
% }
% Despite these affordances, \textit{``little is actually known about the way companies and professionals use and incorporate online user feedback in their development processes."} \cite{van2021role}. 
% The few existing studies of industry practices utilizing user feedback have  found that companies are considering newer evolving feedback channels like social media to improve their feedback collection methods \cite{van2021role} and that processes such as continuous integration could help in the collection of feedback \cite{johanssen2019practitioners}. 

% Thre is little existing guidance on the best practices to manage the ever increasing number of user feedback channels and what determines a high performing organization in this regard. 
%The current research is insufficient in providing a well-defined and formalized process for managing user feedback from various sources to enhance the effectiveness of the feedback management process, derived from comprehensive empirical evidence from industry. 
% Due to the ubiquity of social media platforms \cite{ogink2019stimulating}, it has become useful for organizations to derive requirements from such platforms. 
% For example, social media giant Twitter experienced significant drops in the number of users over proposed changes to the platform \cite{stokel-walker_twitter_2022}, where users switched over to its competitor platforms \cite{rochko_twitter_2022}.
% Another example is when users left Meta products with privacy as a main concern and switched to other platforms with perceived stronger privacy safeguards \cite{statt_whatsapp_2021}. 









%Old related work March 27
\section{Related Work}
% \subsection{Importance of Trends}
% It is critical for organizations to understand and manage current trends in order to maintain a successful business model \cite{granig2020organisational}. 
% Understanding how organizations manage trends in client-feedback and which challenges they face is important to organization-sustainability. 
% According to Parida \emph{et al.}, sustainability encapsulates the management of responsible production such that corporate relationships and social environments are well preserved despite changing demands on a company's abilities \cite{parida2019and}. 
% Preserving sustainability thus helps companies achieve their goals and improve their presence in a competitive market \cite{reim2015product}. 
% Previous work by Parida \emph{et al.} identifies certain trends and qualifies them to be extremely influential as trends impact an organization's methods of initiating change \cite{parida2019and}. 
% So, while the impact of trends is undeniably significant, the need to understand and manage these trends which arise from an immense amount of sources remains as an overwhelming challenge for many software organizations. 

Understanding how organizations manage client-feedback and which challenges they face is important to organization sustainability. 
According to Parida \emph{et al.}, sustainability encapsulates the management of responsible production such that corporate relationships and social environments are well preserved despite changing demands on a company's abilities \cite{parida2019and}. 
Thus, to preserve organization sustainability it is essential that companies consider and understand potentials of user feedback, particularly given the constantly evolving nature of the various sources of feedback.
Previous studies have tried to better characterize user feedback including with the term ``voices of users" \cite{tizard2020voice}, which tries to contextualize all the sources of user feedback.
This concept is extremely powerful, as it reveals many issues present with current elicitation methods. 

\subsection{Voices of Users}
% The term ``voices of users" coined by Tizard \emph{et al.} encapsulates all user feedback expressed through various channels, including social media, thus informing software companies of user needs and concerns. 
% The term ``voices of users" encapsulates all user feedback expressed through various channels, including social media, thus informing software companies of user needs and concerns . 
The concept of ``Voices of Users'' is a more complex topic than simply ``analyzing user feedback'' as it involves the gathering and analysis of feedback from potentially diverse users with different needs, preferences, and expectations \cite{tizard2020voice}. 
This means that analyzing the voices of users requires more complex, intricate processes. 
While traditional elicitation methods are effective to a  certain extent \cite{van2021role}, truly listening to the voices of users helps organizations reap the benefits of effective uses of feedback \cite{van2021role};  thus it is a concept worth an organization's time and resources. Traditional elicitation methods like surveys often rely on a small set of stakeholders or experts to define and prioritize requirements. 
While these methods are needed, they fail to capture the full range of user needs and perspectives \cite{tizard2022voice}.  
Additionally, these methods may not take into account the evolving needs and preferences of users, as they often involve a one-time or infrequent gathering of requirements.

Gathering voices of users can assist software organizations to increase their marketability, thus improving the success of the product as user satisfaction is increased. 
In addition to contributing positively to a product's and thus company's success, the effective management of voices of users could prevent negative events for an organization, such  as loss of resources dedicated towards pursuing the wrong pieces of feedback, or pieces of misinterpreted feedback. 

Truly listening and considering user feedback, especially from a wide variety of sources brings up many complications for interpreting user feedback; one example of this may be considering the culture from which the feedback originated \cite{tizard2021voice}. 
For example, an individual from a more collectivistic culture is more likely  to recommend a software product to friends compared to someone from an individualistic culture. 
In a study conducted by Tizard \emph{et al.} this phenomenon was especially observable when searching for feedback via social media interactions \cite{tizard2021voice}. 
% When taking a moment to consider how many layers there are to each piece of user feedback, it becomes evident that there is a lack of understanding on how to manage this feedback. 
With the current state of knowledge, software engineering teams do not have the processes to receive and interpret voices of users, correctly interpret it within the scope of location, culture, and various other demographics, and thus risk implementing the wrong changes, or overlooking critical feedback. 

\subsection{Organizations and Social Media Engagement}
With an increase in social media engagement, users are generating more \textit{narratives} in their user feedback around software products \cite{li2022narratives}. 
However, managing all the trends that these narratives give rise to is a very complex task, and requires an understanding into what practices are currently employed in software organizations. 
Recent work analyzing the way practitioners consider user feedback suggests that there is a lack of interpretation of implicit feedback \cite{johanssen2019practitioners}. Explicit feedback on the other hand, was extremely popular in industry, with a significant dependence on manual approaches to gathering feedback such as surveys or emails \cite{johanssen2019practitioners}. 

While explicit feedback gathering methods have been widely used and relied upon, it prevents the facilitation of truly continuous development, as the feedback is gathered in distinct periods as opposed to continuously in parallel to development. 
Johanssen \textit{et al.} even suggest the integration of continuous user feedback capture as it has the potential to diversify the requirements organizations work with. 
These findings leave us wondering how we can better pay attention to implicit sources of user feedback, and what strategies may mitigate the challenges associated with this task. 

One major source of implicit user feedback is social media. Looking through trends on platforms such as Reddit, TikTok etc. are as close as developers can get to eavesdropping into private conversations to gather feedback and honest opinions. 
Recent research suggests that growing social media platforms are catalysts for new innovation in organizations \cite{ogink2019stimulating}. 
Previously, it has been found that organizations with presence on less social media platforms also had the smallest proportion of feedback coming directly from users, which contradicts current recommendations to listen directly to the voices of the user's \cite{wiegers1997listening, 9218201}. 
Furthermore, considering more online channels for feedback helps developers gain a more comprehensive picture of what their end-users need \cite{9218201}. 
Despite the benefits of using social media for deeper insights into user feedback, a previous study revealed that while 9 out of 11 startups look into social media for a competitive edge, larger companies only loosely track their social media presence \cite{10.1145/1984701.1984702}. 
This suggests that many companies are not grasping a comprehensive view of the requirements expressed by their users, and are developing products that may not serve the true needs and wants of their clients.

% User feedback is a highly critical aspect for software organizations to consider as part of building new features and resolving bugs.
% Social media user feedback, a growing segment of user feedback, has great potential to influence user behavior, which may in hindsight impact whether users continue using a software \cite{li2022narratives, voramontri2019impact}. 
Despite the efforts of various studies to learn about the use of user feedback in the industry \cite{van2021role, johanssen2019practitioners}, there is still a lack of empirical evidence on the best practices for managing user feedback, especially social media feedback. 
To address this, we embarked on this study with the goal of reaching out to industry practitioners to gather insights on whether software organizations even consider user feedback, particularly social media, and if they \textbf{do} consider this feedback, what are the actions they exercise to manage these user feedback.
% Our 40 interviewees from 32 organizations confirmed that understanding user concerns, especially from social media, is critical to their product management.
% Our interviewees also highlight the perils of not considering or misunderstanding these user concerns.



% \nowshin{Summarize Guzman and Johanssen paper}
% While studies have investigated the industry practices of user feedback utilization, they are mostly focused on how and why feedback is collected and what are the challenges that practitioners face.
% they have either reported the practitioners perspective on the importance of collecting feedback and the challenges encountered by practitioners during this process, particularly the time-consuming nature of the feedback collection process \cite{van2021role}. 
% they have either reported the practitioners perspective on the importance of collecting feedback and the challenges encountered by practitioners during this process, particularly the time-consuming nature of the feedback collection process 
% Similarly, another study presented an overview of the different ways that practitioners collect and utilize user feedback. 
% However, they only reported the overall view of the feedback collection process in terms of when and how feedback is captured and what is the best way to collect feedback, 
% They also add the reasons for feedback capture.
% They reported that capturing feedback from people inside the company was found to be beneficial, 
% Hence, current research lacks to describe a formalized process on how feedback from different sources are managed, processed and sent to development and what are the best practices that would make this feedback management process most efficient. 



%Active response old
% The company needs to adopt fast decision making processes.
% This involves streamlining the process of collecting, and validating feedback to enable the swift roll-out of critical features or bug fixes.
% For an organization to have the best possible active response time, organizations must expedite the initial steps of the development lifecycle and aim to deliver essential updates within a short timeframe, such as one or two weeks. 
% This enables companies to label themselves as high-performing entities that can quickly respond to market demands and customer needs.

% \begin{table*}[t!]
%     \centering
%     \setlength\extrarowheight{-10pt}
%     \begin{tabular}{p{0.6\linewidth}p{0.20\linewidth}p{0.12\linewidth}} \toprule
%      Raw Quote & Code(s) & Theme \\ \midrule
%       \textit{If it's [affecting] the ability for somebody to log into their email, just as an example, [we] don't need to look at data to know that that is a high priority, kind of a showstopper issue, and it needs to be addressed immediately. However, for other issues that are [sic] issues, still important, but, [sic] maybe affecting fewer people. That's where we'll kind of lean on data to help us decide what to prioritize now.}    &  Prioritizing, \par FeedbackfromSoftwareUsage, \strut	 	MethodsToAnalyzeTrends,	IdentifyingTrends    & \textbf{Prioritizing User Feedback}  \\ \midrule
%     \end{tabular}
%     \caption{Conversion of a Code from an Interview into Code and then into Theme}
%     \label{tab:quote-to-theme}
% \end{table*}

% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=0.95\linewidth]{figures/ResearchDiagram.pdf}
%   \caption{Research Process}
%   \label{research-process}
% \end{figure}



Active data collection:

% Our participants emphasize how all sources are critical in understanding the different aspects of the user perception.
% The successful companies always proactively seek feedback from multiple sources. 
% \qs{We have like millions of users that are using a product. And so usually we interact with them through social media, or they use the block channels that we have, we also have a specific [tool] ... they can just like put [the feedback] on the [tool], and then all other users can come there, they can see that ideas, they can vote on it or and comment on it. So I think the community is definitely the first look that we have to see what users really need and the first layer of feedback that we look at. ... The second one is that within the [tool], we have a group of people that sits between the customer and our team, and they interact with our like, top enterprise customers that are paying. So, that's like the top 100, top 50 enterprise customers that are using our product. And, so with those types of customers, we have like regular interactions like either on a weekly or monthly basis to just make sure that those customers are unblocked. And of course, since they are like they are heavy users of our product and paid with money.}{P25}
% The small and medium companies that we interviewed were also in agreement to considering various sources.



Results V.1
\section{Study Results}
In this section, we provide an in-depth analysis of the findings obtained through the research methodology employed in this study. 
The research questions posed earlier are answered and discussed in light of the data collected.
% Findings 4.5
% RQ1 1.75 -> currently 2.5
% RQ2 2 -> currently 3 
% 0.5 is taken up by pipeline figure
% RQ3 0.75 -> Dunno

% Discussion 1.5
% 1.5

% Collection of Data: Put the table
% find if there is something that's new in this section from literature expand on social media aspect compare with the current research. Highlight what we're doing and what previous research has done

% Previous study suggests that social media influcences user behavior on software. Do organizations care about it? 

% RQ2 revamped:
% Dive deeper into each part, add details, add lit review



\subsection{What are the different sources that formulate the ``voices of users''? (RQ1)}
``Voices of the users'' is the collective of user feedback and opinions expressed through various channels, informing software organizations of their needs and expectations to enhance the overall user experience \cite{tizard2022voice, tizard2020voice}.
When it comes to managing these ``voices of the users'' or user feedback, the first critical aspect is identifying where and what to look at. 
This requires identifying the community of potential and current users of a software, product, or service. 
Our participants described a variety of sources that capture user feedback from the \textit{community}, which include \textbf{\emph{emails, phones calls, video conferencing, product forums, support tickets, social media (e.g. Reddit, Twitter, Facebook, and YouTube), app reviews, user workshops, user interviews, surveys, and usage metrics}}.
Given this variety, we split these into three categories: conventional user feedback (inbound and outbound), usage metrics and social media sources.
In this section, we describe how software organizations utilize the three sources of user feedback by addressing the sub-RQs.

\subsubsection{How does software organizations leverage conventional sources of user feedback? (RQ1.1)}

To collect user feedback, organizations employ both inbound and outbound methods, which typically involve individuals in various roles such as product managers, customer support manager, customer success manager, and QA analyst, etc. who are responsible to facilitate the feedback mechanism.

\noindent\textbf{Inbound Feedback:}
One of the most common types of user feedback is inbound feedback \org{1-5, 7, 9, 10, 12, 14-25, 27, 28, 30-32}. 
It may take the form of emails \org{1-32}, phone calls \org{3, 4, 6, 7, 9-11, 16, 22, 25, 28, 30}, video conferencing \org{3, 4, 7, 20}, support channels \org{1, 4, 5, 9, 10, 13-25, 27, 28, 30-32}, and app reviews \org{17, 22, 25, 26, 27, 28, 30, 31 }. 
In these examples, users can use these channels to directly contact a software organization when they need assistance from customer support for something that likely does not work. 

Some organizations create their own community forums \org{4, 6, 8-11, 18, 21, 22, 30, 31} to gather feedback and engage with customers. 
\qs{[Online community forum] is kind of like open source feedback. We can go in, you can ask questions, and you can upvote different feature requests.}{P10} 
Platforms such as Slack are also used by these organizations to collect user feedback collaboratively. 
However, as described by P6, these sources may have drawbacks, such as low participation rates or users not filling out feedback forms.

For software organizations that develop mobile applications, staying on top of major changes to the underlying operating system or phone version and monitoring user reviews on Google Play Store and Apple App Store are crucial for anticipating impacts on users and directing product development. 
\qs{We would always watch the app store when a big iOS release would go out, or a big Android release... we would all watch the feedback...it'll give you a pretty good feel for one of those two things, the new version of the app or new version of the operating system. [What] caused the app to not be driving the same level of sentiment.}{P36}

While it should be acknowledged that not all feedback sources are relevant to every organization, gathering feedback through inbound phone calls, emails, product forums, and app reviews is critical for developing successful products and enhancing user satisfaction.

\noindent\textbf{Outbound Feedback:}
Outbound feedback refers to the feedback that is actively sought by the software organization \org{1-13, 16, 20-23, 27-31}, rather than waiting for users to provide it on their own. 

A popular outbound method practiced by many organizations includes sending out automated emails when a new version of their app is release to gather feedback. 
However, as echoed by P13, to be more proactive, organizations also offer users the opportunity to book feedback sessions with the product manager.

Our participants emphasized the significance of face-to-face meetings with users as an extremely valuable feedback source, highlighting it as one of the most effective methods for obtaining feedback.
Large and resourceful organizations often utilize user workshops \org{11, 28, 29, 30} in research labs, where users are invited to test software products, while the organization observes and analyzes the users.
% \qs{There are a team of people that would actually ask the public, the public obviously need to sign NDA, if they're exposed to some part of the [product] that's still on research. Then [we] basically record these sessions and watch how they do.}{P38}
As described by P37, these user research labs, equipped with advanced technologies such as eye movement trackers and ceiling-mounted cameras, are very expensive. 
Conducting these user workshops whether in the form of focus groups or interviews is also time intensive and require specific research roles that are not accessible for many organizations. 

In some instances, organizations would go out to the public, such as coffee houses and ask people to use their software products.
\qs{We would go to coffee shops. We'd sit there maybe with a computer and [something] to show about our [website] or maybe our [app]. And just talk to users and say, ``Hey, we're thinking about doing something that does blah", and just literally just have a conversation with users about, oh, this is a cool idea. ``Here's what I think you should do. I saw this somewhere, maybe be cool."}{P36}
The central benefit of the direct user interaction is that they facilitate observations and analysis of users utilizing a software product.  

Outbound feedback obtained through a variety of methods, can complement inbound sources to help organizations proactively gather feedback from their users and use it to improve their products and services.

\subsubsection{How does software organizations leverage software usage metrics as a source of user feedback? (RQ1.2)}

When it comes to user feedback, user metrics from software usage can provide valuable insights for software organizations. 
Our participants from 26 companies reported that they collect some form of usage metrics to track how users interact with their software product. 
However, participants from the remaining 6 companies \org{9, 12, 15, 18, 24, 32} noted that their companies either have robust testing processes \org{24}, work with large customers \org{9, 15, 18, 32}, or have not yet integrated the necessary tools and processes to collect user metric data \org{9, 12}.

We found that user usage metrics are an important source of insight for organizations of all sizes, including small, medium, and large organizations, when it comes to understanding user behavior.
P2 describes using tooling to record, \q{how many people stay and how many actions are doing you can play, what they are doing on your platform. So where the mouse is going, where they are looking at, how much time they spend on a specific feature. And that's going to help you understand how people are using a product. So it really shows you what people are doing.}
We also observed organizations heavily relying on user usage metrics to triangulate with inbound and outbound user feedback.
\q{There's always going to be people who encounter issues, but don't reach out. Customer usage data from what we gather on our back end [paired with] continuous communication with a support team to advise us on what they're seeing, and what what is most popular}{P13}

Collecting usage metrics is only one part of the feedback gathering process, as organizations also need to have a dedicated team of data engineers or data analysts to thoroughly analyze and interpret the data.
However, incorporating user usage metrics into a feedback loop can provide software organizations with valuable insights that can help them make informed decisions and improve their products for their users.


\subsubsection{How does software organizations leverage social media as a source of user feedback? (RQ1.3)}\hfill

\noindent\textbf{Monitoring Social Media:}
In today's digital age, social media plays an important role as a public square for user discourse about software products. 
Social media has emerged as a crucial tool for organizations to connect with their users and gather valuable insights about their needs and preferences, representing a new and powerful outbound feedback gathering source. 

% A key aspect still imperative throughout the validation step is that it is important to focus on trends and themes rather than individual comments. 
% It is simply not feasible to respond to every single piece of feedback, so organizations need to look for patterns that indicate broader issues. 
% One effective way of doing this is by taking a random sample of users or targeting those who are highly engaged with the product or service.
% \qs{You don't need to look at every single [comment] because a trend occurred. You just take a random sample of the users, and sample based on some level of engagement that makes it a bit more useful.}{P1}

Our participants discussed how their organizations monitor a variety of popular social media platforms including Twitter \org{1, 2, 5, 11, 13, 17, 18, 22, 24, 25, 29, 30}, Reddit \org{1, 2, 12, 16, 17, 19, 21, 22, 25, 30 }, LinkedIn \org{7, 12, 21, 23, 29}, Facebook \org{17, 19, 27, 31}, Instagram \org{1, 17, 20, 31}, Discord \org{1, 2, 5}, YouTube \org{1, 23, 30}, and TikTok \org{17, 25}.
From Reddit to TikTok, proactive organizations are constantly monitoring their online presence to determine what people are saying about them. 
These conversations reveal the potential bugs and features that may impact these organizations, big and small, in various industries.

For example, in one interview, a participant revealed how at their organization, they have a dedicated team who monitors social media feedback on Reddit. 
% \qs{There is a good amount of social media involvement in the Reddit posts... Not only PMs, I think there are a couple teams that are dedicated to look into those. Always. 
% They always check and we get monthly emails what are the users talking about? What do they like? What do they don't like? Like, I know that there is a [product] feature that users really love, they're always talking about it that they love that.}{P26}
\qs{We have a team that just looks at social media, and they report on like, the biggest \textbf{trends} coming from social media.}{P27}
This feedback helps the team identify issues and features that users like or dislike, and monthly emails are sent out to report the findings. 
In essence, the trends that emerge from large volumes of feedback on social media serves as a useful part of product and engineering teams.
% \qs{We have a team that just looks at social media, and they report on like, the biggest \textbf{trends} coming from social media.}{P27}

Similarly, an interviewee from the gaming industry revealed how social media monitoring is essential for live games. 
P32 explains how their product managers monitor Twitter and other social platforms, to receive real-time updates on user concerns and bug reports related to their live game. 
They quickly engage engineering teams to address these issues to ensure the best possible user experience.
% P32 explains how their organization utilizes Twitter and other social platforms to receive real time updates on user concerns and reporting on bugs.
% \qs{People tweet. So there are different channels they [talk]... Our [product managers], they monitor those channels. Because [redacted] is a live game, if something is impacting the people, [they] complain in those channels. And we see that.}{P32}
% The organization's product managers monitor various channels to identify issues that impact users and quickly engage engineering teams to address them. 

We found something that is unique to the gaming industry is the impact that ``game reviewers" have in driving a trend that goes viral on social media.
These trends could snowball and force these software organizations to respond.
\qs{We look at a lot of different sources... Twitter... Reddit is another common one... \textbf{One YouTuber} [highlighted this]. In [redacted], there are these things [features that] players could pick. For this year, the game team decided to revise how the system works?...So there were a lot of negative feedback from the community through public channels talking about [it].}{P38}
Social media feedback is just one of the many channels used to ensure that the game runs smoothly and meets user expectations.

To gain insights from their respective ``communities", our interview participants went to great lengths to uncover feedback from social media.
\qs{I'm asking questions [on Discord]. And generally I don't ask question under my name. I have some fake names that I use... So I have some fake name with a male and a female account question because [sic] you need to [reduce] bias. Some guys want to seduce a girl and some guys are gonna be aggressive with [me]. So I'm basically trying to have neutral data points non biased, you always going to have bias, but your goal is to reduce bias.}{P2}
To mitigate against potential biases that users may express in online social media, this participant not only uses pseudonyms, but also converse with their community via female and male profiles.

However, social media monitoring is not just about gathering feedback. 
It is also about identifying trends and staying ahead of the competition. 
\qs{One of our competitors, [they're] on LinkedIn. And [they] just leak information all the time. [They] posted a link to their internal feature requests... I was like, ``Oh, thank you very much. I'm gonna take a look at all the information you have here. And we're gonna pull it down from this, because it's public."... So now I can turn around and have our marketing team create a marketing push.}{P14}
Companies have to be able to react quickly to changes in the market and adapt their strategies accordingly. This means monitoring not just their own brand, but also their competitors.

Social media monitoring is a crucial tool for businesses of all sizes and across various industries. 
It provides real-time feedback from consumers, helps identify trends, and allows companies to quickly address issues and improve their products. 

\noindent\textbf{Limitations of Social Media}
While our participants immersed us with examples of their collection of feedback from social media, they also listed some limitations associated with feedback from social media that need to be addressed.

When feedback from social media is collected, the quality of feedback from users should be scrutinized.
Social media feedback can often be vague and lacking in detail, making it difficult for organizations to get an accurate picture of a problem or feature. 
\qs{The problem is the quality of the feedback from customers. It is very different from when a customer would reach out and fill out a form of support form. Those types of tickets are more reliable type of feedback compared to social media. Social media, they're often vague... ``It's not working at this account," but, "What is not working?"... There's a lot of details that are missing from that [social media] interaction.}{P11}
This is why an organization may need to reach out to users and ask them to fill out additional surveys and/or interviews to gather more information.
\qs{So you'll notice that some companies would then reach out to the customer and say, ``I can [help] you, thank you for reaching out, can you fill up a form so that we know you're real and you can give us more detail about the problem so that we can solve it?"}{P11}

Another challenge associated with user feedback from social media is the amplification factor. 
Pure volume-based analysis may be misleading, as social media can amplify certain features or conversations, regardless of whether they are valid signals or not. 
This can lead to misinterpretation of trends, and companies need to be aware of this when analyzing social media data.
As explained by P1, \q{I think that a lot of times, when you're doing just pure volume based analysis, you run into that problem, because social media has a huge amplification factor that you have to be aware of. If someone starts talking of a particular feature, more people will start talking about that feature, or more people will start talking about a particular thing.}

Related to the amplification factor is the potential for noise that organizations can collect as part of the feedback.
Sometimes you see a bunch of complaints, but these complaints are not directed at the software product and instead some unrelated aspects.
\qs{Facebook was [used]. And I would say, people used to complain a lot. I mean, like, whenever people, things work fine. People don't compliment in [Facebook]. But the thing is [the] majority of complaint was actually unrelated to us. Because most of the time, it was complaining about [something unrelated].}{P34}

From social media, some interviewees expressed that bugs are widely reported, but feedback regarding on feature requests are more scarce overall.
\qs{We noticed we only got negative feedback through social media or like positive reviews. It was never feature requests. It was mainly someone's having an issue with a bug, or they just really liked the product.}{P17}

Based on our interviews, we found that many small, medium, and large organizations use social media feedback in some capacity. 
One of key limiting factors to more widespread adoption is that it is currently quite ad-hoc, with no formal way.
Even in large organizations where they may attach dedicated teams to collect social media user feedback, this is conducted through manual means.
\qs{There's also no tooling that we have [for] social [media]. [Nothing] we [have] to actually catalog [and] count that. An incredibly manual process for someone to actually sit down and read everything and try to code it in a way that we could do something with it.}{P35}

Despite the aforementioned challenges, ultimately, a lot of users will choose to join and leave a software product depending on perception of the product and trends on social media.
As explained by P24, \q{A lot of business will come from reputation. Whether people recommend and stuff offhand. ``Oh, you should use this, or this is really useful for this sort of thing." So social media can either enhance or damage your reputation, and that will directly affect the business in many cases}.



\subsection{How do software organizations manage user feedback? (RQ2)}

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.95\linewidth]{figures/VoiceofUsers.pdf}
  \caption{The Generalized Data Flow of the Voices of Users. \\ (A) represents the data flow of the ``Voices of Users". (B) represents the life cycle of user feedback as part of software development process. (C) indicates the 3 categories of user feedback that formulate ``Voices of Users". (D) indicates the transformation of user feedback throughout different stages of the user feedback life cycle.}

  \label{voice-of-users-data-flow}
\end{figure}

Once an organization identifies and collects a stream of user feedback from a variety of sources, the next fundamental step is managing this trove of feedback.
Our interviewees come from diverse software industries and organizational sizes, but they share commonalities across the management and usage of user feedback. 
For an organization that strives to understand its user requirements, perception, and areas for improvement, it should adopt methods to listen to the \emph{``Voice of the Users"} as well as effectively managing it. 
We captured these commonalities and present them in a generalized data flow 
of the \emph{``Voice of the Users"} in Figure \ref{voice-of-users-data-flow}.
In the following subsections, we describe in details the main steps in managing user feedback 1) analysis, 2) validation, and 3) prioritization.

\subsubsection{Analyzing User Feedback}
Analyzing user feedback is an essential part of understanding user concerns and requirements to develop successful products and services. 
It allows product managers, developers, and senior managers alike to gain a deeper understanding of user needs, preferences, and pain points, enabling them to make informed decisions about product features and bug fixes.

The main purpose of the analysis of user feedback is to find emergent trends and common themes that develop from the user voices. 
Part of the process is listening to the bastion of user voices and group similar patterns.
\qs{What are the things that they struggle with. [We] went through all that feedback and grouped the similar themes about what were the common complaints and and what were the common dream features that everybody wanted.}{P4}
The same question repeated again and again is often representative of a underlying problem. \qs{The number of times the question was raised was also important, because that means many, many [users] are having this confusion.}{P5}

Our interviewees all shared with us the importance and main goals of finding the ``themes" in the feedback.
\qs{Ultimately, it's about the themes. It's looking for other patterns in the comments... We released a new version that was 100\% deployed in the App Store. All of a sudden, we're starting to get some some tanky reviews and people complaining that [redacted] are slow. Because you know, you're always looking for something to appeal to, to the large majority of people.}{P36}
When customer complains through support channels, the volume of complaints can illustrate trends as well as explained by P14, 
\q{You got a trending amount [of] support tickets complaining about a specific issue.}
An organization cannot expect to satisfy every possible user out there, so identifying the common themes will help uncover the potential bugs and features that matter for the masses.


However, analyzing user feedback is not a straightforward task, and there are several important considerations that must be taken into account.
One key point that emerged from our interviews is the importance of balancing high-level feedback with detailed feedback. 
As P27 noted, if an organization wants to dive deep into an area, then one-on-one interviews or sessions with small groups of users are necessary. 
This type of feedback allows product teams to gain a detailed understanding of how users are interacting with a particular feature and whether it is providing the intended value. 
In contrast, P27 notes that high-level feedback in the form of NPS or thumbs-up/thumbs-down ratings can provide a quick and easy summary of overall success. 
Both types of feedback are necessary for organizations to make informed decisions and push a product forward.

When an organization takes the advantage of social media user feedback, it can provide rapid insights on bugs the occur.
\qs{During the testing process. We missed [including the menu items]. We woke up one day... All these messages on social media being, ``what the heck, I just updated and none of the menu items [exist] anymore." }{P13}
We see the importance of pure volume of feedback manifesting as a key factor of identifying themes.
% \qs{People will post snapshots of a Reddit post with a whole bunch of votes. And [users are]  mad about the seat heater, or on the new UI. And then a month later, there's a JIRA ticket and someone's working on it. So}{P22}
For organizations that dedicate the resources to monitor social media, our interviewees explained the importance of paying attentive attention.
\qs{On Twitter [and] LinkedIn, there's a ton of different accounts that are out there. [We] monitor those. And I also know that anything that I say on social media that has anything to do with [our product with] a hashtag, they [will] pay attention to that. We [also have] Instagram and [are] aware of people send their feedbacks and based on that [our] team [will] decide whether to develop the feature or not.}{P38}

However, P38 also points out that it's essential to balance the signal-to-noise ratio and consider which groups of users are over-represented or under-represented in this type of feedback. 
After all, some groups may be more likely to post on social media than others, which can skew the data. 
It's important to ensure that the feedback received represents a diverse range of users and is not biased towards any particular group.
Identifying themes can also be tricky and onerous, as P18 explained there is a lot of manual reading of user comments and organizations may not actually understand what users are saying.
Based on conversations with our interviewees, disseminating themes from user feedback is still an overwhelmingly manual and laborious process.

Furthermore, analyzing user feedback requires an understanding of the limitations of the data. 
Users may have conflicting opinions or report pain in the spur of the moment.
\qs{A lot of the time, requests come in, they're not flushed out fully. In the moment, they're frustrated with something. And then two hours later, [they] don't need that}{P14}
It is crucial to listen to all feedback, but it is equally important to recognize that not all feedback is equal.
From analyzing user feedback into themes, organizations can gain a deeper understanding of their users and pick out themes that represent important features and bug fixes for future product iterations.

\subsubsection{Validating User Feedback}
The next step after analyzing user feedback and identifying themes is validating those themes that emerge. 
In particular, how does an organization know that a specific user feedback is valid or worthy of action?

The potential consequences of misinterpreting themes are significant. 
\qs{The movie Morbius became a meme... The core of the meme was that no one had actually seen this movie. [Discussion] became very popular. Sony actually extended the theatrical release of the movie, because they saw a trend that the popularity of the movie was increasing. They did not test to determine that the reason why the popularity of the movie had increased is because people were having fun talking about how no one had seen or any intention of seeing the movie.}{P1} 
The end result was that the company wasted the money re-releasing and re-marketing the movie to no audiences \cite{mendelson_box_morbius}. 
Misinterpretation is particularly pronounced for user feedback on bug reports. 
A reported bug may be in reality a misunderstanding.
\qs{You first got to validate whether it is actually a bug or if it's intended design, sometimes customers will misunderstand the system. They'll file bugs against things that are designed as intended.}{P24}


The lifeblood of validating user feedback involves triangulation between all the sources of user feedback to reduce misinterpretations. 
26 out of the 32 organizations studied collect at least some form of user metrics which it critical to the triangulation of user feedback themes.
One can compare the themes from with conventional and social media sources with user usage metrics and vice versa. 
% Analytics are key to understanding user behavior and identifying potential areas for improvement. 
By tracking user engagement with different tooling such as Hotjar or Google Analytics, we can see which features are being used effectively and which ones are being ignored. 
These tools are sophisticated enough so that anyone at the software organization could replay a user usage session like a movie and visualize every button click, mouse hover, and delay on page. 
\qs{Everything is tracked, every click is [tracked], every action is tracked. That user feedback is how users interact with the [product].}{P39}

However, analytics can only take us so far, and organizations need to supplement this data with direct feedback from users.
\qs{We check analytics to see like who's using what, and then if someone's not using it follow up with customers and do a review.}{P7}
Similarly, 
\qs{Every big system has monitoring. So we will align that [with other sources]. [We see] people are complaining that they cannot log in and we will see in our graphs and charts. ``Oh, yes, the services down."}{P32}
The triangulation process most typically would require coordination from multiple teams as data teams must communicate findings from user usage metrics with findings found from product, customer support, and customer success teams who are more closely in touch with conventional and social media sources.
Establishing tools and processes to support this triangulation would require efforts, but the rewards for an organization is that has greater likelihood to verify which features and bugs are relevant and impactful for users before dedicating valuable engineering and product hours.

Triangulating user feedback may open new collaborations and communication channels with cross-functional teams as different teams share responsibility to validating user concerns. 
\qs{I have to bug [product people] often [for] validating because there are customers that are louder than others, you have to factor in that they could just be one very squeaky wheel. If one customer complains about it, there could be a myriad of customers behind the screen who haven't said anything about it, but it is a problem for them. So using data to validate.}{P12}
One possible strategy is starting with social media to identify themes and then directly contacting users to validate. 
\qs{Social media is a good place to get started. You find a trend. Next step is to collect a statistically relevant, smaller sample of genuine accounts that you care about.}{P1}

Validating user feedback is an important process with the end goal of using triangulation to mitigate misinterpretation and misunderstandings.
After this process, an organization would have collated a list of feature and bug concepts that were validated and represent genuine issues. 


\subsubsection{Prioritizing User Feedback}
Prioritization is a crucial step in the generalized data flow of the voices of users, which involves making trade-offs between different bugs and features to maximize benefits for the organization. 
% These trade-offs are made given that organizations, particularly small and medium sized ones often have limited development resources. 
% Striking the perfect balance between trade-offs and identifying the most paramount feature and bugs is essential. 

As per our interviewees, the critical factor to prioritization is whether features and bugs match a company's vision and goals. 
Best described by P27, \q{if we get feedback, that doesn't align to anything we're doing.. [if] it's not something that we're going to address this year, we're not going to redesign it, we're not going to revamp it.}
That is not to say that they would completely ignore it, \qs{I'd probably look at little quick fixes I could make [it].}{P7}


The key to prioritization is balancing trade-offs so that there is mutual benefit for the users and organization. 
P6 astutely observes, ``if they [users] are giving us [feedback], it's likely...that [something] would help them. [They] help us because they are going to use our system."
However, not all feedback is created equally and the often ad-hoc process of prioritizing can result in the wrong decisions, which is particularly troublesome for smaller organizations with limited resources. 
\qs{Sometimes we end up choosing such a [feedback] to implement, which probably just takes a lot of time and we have limited manpower. [Alternative] task which [ended up] more important gets delayed. So we do make mistakes, but we try to avoid that by discussing and analyzing [if feature is] gonna contribute.}{P6}
% Using one judgement to determine priority is echoed by P22, \q{it's just a matter of using your judgment, your best judgment is enough to determine priority... Have a clear discussion with your team and [say] this is important because XYZ and I'm gonna work on it now.}

Furthermore, the underlying driving force for major features is often the revenue that a prospective feature may bring to the organization.
\qs{At the end of the day, we need to make money. If there is a feature that one customer wants and [has] a significant impact on revenue, we're going to implement the feature. [The] features need to be reasonable. If they ask to put a pink elephant on the homepage, we're not gonna do that. But if they implement a feature that's gonna benefit [many] people. Yes. We're gonna do that. But it needs to drive revenue.}{P2} 
% There may be limitations in terms of budget or resources and this shows that even if the feedback is important, it may not always be possible to act upon it immediately.

When prioritizing tasks, the company places emphasis on activities that generate revenue or prevent financial losses, while also factoring in practical considerations.
% \qs{In the current economic condition, the company always is prioritizing things that make us money and prevent us from losing money...[But] there's significant delay between feedback and effect... [May] take a month or two to really show.}{P28}
This means that even if feedback is prioritized, it may take time to see the results, but an organization can \qs{find small issues quickly and fix them.}{P28} 
Such approach was corroborated by P30 who explained that small feature requests may be approved at the team management level, while larger feature requests may require approval from C-level or other senior executives.

Nevertheless, it is not just about the financial impact. 
As another participant pointed out, \qs{people's perception of the company as a whole}{P28} is also an important factor. 
If the feedback is related to something that is damaging the company's reputation, it will be given priority even if it doesn't have a direct financial impact. 
After all, a company's reputation is invaluable and can influence user behavior to adopt or drop a software product. 
%Add our citation

Furthermore, when it comes to trade-off between bug fixes and features, different levels of priority are assigned to them based on their criticality and the team's assessment of customer impact.
One assessment strategy from P31's experience is creating Jira tickets with points allocated, and the intensity is calculated based on customer-facing teams' feedback.
\qs{New features are typically lower priority than bug fixes. So usually bug fixes are prioritized top of the list, because it's something that the users are paying for or having issues with as compared to something that just doesn't exist.}{P17}
% However, not all bugs receive this priority, as P25 conveyed, ``Even bugs also get like priority labels on them." This priority is dependent on number of affected and affect on revenue, but high priority bugs get fixed immediately, where as small bugs may linger for a long time.


Prioritizing user feedback is a necessary step that requires balancing trade-offs for features and bugs.
By striking this balance, an organization may create software that not only meet user needs but also align with their larger vision and goals.

\subsubsection{Development and Release}
At this point, an organization should have identified initial themes based on user feedback, developed feature or bug concepts based on the user feedback through validation, and prioritized the important features or bugs.
The last step of the data flow of the voices of users is the development and eventual release of new features or bug fixes from an organization's prioritized list.
This is the point in the data flow process, where the technical team is given the most responsibility to take the prospective feature or bug fix and develop the software to match user requests. 
When an organization finishes development and the new version of the software passes all the assigned tests, the organization will release the software to its users at the next opportune time.
Depending on the organization, this interval could range from minutes to months. 
However, when that new software version is released to users, a new cycle of the data flow of ``voices of users'' is triggered and new user feedback, good or bad, will makes its way to product managers, developers, customer support staff, data scientists alike. 


\subsection{How does ``voices of users'' fit into product management? (RQ3)}
In addition to understanding data flow for the voices of users, our interviewees helped share insights on the relationship between use of voices of users in requirements engineering and product management practices. 
From our interviews with participants, we identified three main points that organizations should consider for product management. 


\noindent\textbf{Individual Empowerment:} The first point we found is that large organizations \org{O19, O21, O22, O27, O31} often heavily encourage their employees to take the initiative, particularly for identifying issues in the software products.
\qs{There's a lot of ownership among devs. If you're working on something, it's expected that you own that and see the potential risks and impact of you're doing and make design decisions for that.}{P22}

Employees who are invested in the product may pick out themes in user complaints on social media while browsing,
\qs{High majority of [redacted] employees are also very interested in [redacted]. It's very common that the employees will frequent [redacted]'s subreddits. [Some] bug reports and feedback comes from internal employees being on [redacted] related social media.}{P22}
Therefore, employees frequently will post screenshots from social media regarding popular concerns that impact the product {[We see] screenshots of a Facebook post saying ``what does this alert mean?" And then someone's on it, trying to make the customer facing UI more understandable or adding something to the user manual. This \textbf{initiative} is definitely led by employees that have other jobs that just happen to be also invested in these kinds of things.} 

In contrast, we observe some smaller or medium sized organizations having more traditional top down approaches to dealing with voices of users.
\qs{Yeah, the product owner would decide the prioritization of what the backlog looks like. And then in their sprint planning meetings, they would pull it into work to be done. I do not let the developers decide the priority.}{P14}
We found that founders or senior managers sometimes institute a separation of powers.
\qs{I think [once] the product team kind of has their vision as to what exactly it is that they need, then they'll start pulling the technical team because there's no point pulling us in any earlier than that until they know what they actually want.}{P15}
However, we see the benefits of individual empowerment when it comes to addressing the voices of users.
In particular, the empowerment and mobilisation of all employees provides more overall support to product management. 

\noindent\textbf{New Age Resource Allocation for Product Management}
Another new aspect that our participants highlighted is the importance of having a dedicated role or team to disseminate all the various user feedback sources. 
This aspect starts with the increasing reliance on user usage metrics as a key source of feedback. 
Despite data scientists and data analysts roles becoming ubiquitous in software organizations, the volume of data is vast.
\qs{You have logs for everything. There's almost too much data. I think that one of the biggest issues is who's interpreting the data who's making the dashboard.}{P22}
This means that these organizations must allocate resources to not only collecting user feedback, but also interpreting the data. 

Related to this is the importance of having a dedicated team to collect and manage social media feedback in an organization. 
Our participants highlighted that most organizations have marketing or public relations teams that manage source media sources, but the process for coordinating this feedback is still primarily ad-hoc at the moment. 
This problem is exacerbated if an organization wants to conduct rapid feedback analysis on the social media data via sentiment analysis or other techniques. 
\qs{You [have] some marketing team. It might not be even one person. [This team] is in charge of gathering those sentiments and feedbacks and then making sure that we are not losing any valuable feedback}{P32}
Organizations may also benefit from roles that are cross cutting in nature and who understand the various sources of user feedback such as a customer support agent who has knowledge about user usage metrics in addition to conventional user feedback sources. 

Our interviewees further address the need for tools in a company to gather feedback and insights about products and services. 
\qs{lots of ideas can come from the social media post. I don't know if this kind of tool is available in the market or not?}{P20}
They also highlight that the absence of tooling in social media makes the process highly manual and time-consuming. 
\qs{There's also no tooling that we have in social in order to actually catalog that count that, and it would be an incredibly manual process for someone to actually sit down and read everything and try to, you know, code it in a way that we could do something with it.}{P35}
As a whole, our conversations with the participants reinforced the importance of resource allocation within an organization whether in the form roles or tooling for product management. 







\subsection{Data Analysis}
The analysis process comprised of few different steps.
The process started with the interviews, where the questions evolved with each participants answer.
We recorded each interview and transcribed them using an automated transcribing tool and manually verified them.
% Afterwards, we conducted thematic analysis method proposed by Braun and Clarke \cite{braun_using_2006} which required the research team to follow these steps: (1) initial reading of data and familiarizing, (2) identifying initial codes, (3) generating themes, (4) reviewing themes, (5) defining themes, and (6) creating a report.
We utilized an inductive approach \cite{corbin2014basics, cruzes_recommended_2011} to identify the initial codes from the raw data related to industry practices for utilizing user feedback in their software development process. 
% An inductive process requires reviewing of the data line by line to find obvious concepts and assigning codes based on the concept. 
% This approach uses `constant comparison’ method which allows the researcher to refine the codes through extensive reviewing, specifying and comparing texts that matches the concepts \cite{corbin2014basics, cruzes_recommended_2011}. 
% Following these steps, we began to identify multiple codes from the transcripts.
% Each transcript was first coded by one research member and then validated by a another member to reduce potential bias through constant discussion and peer debriefing \cite{nowell_thematic_2017}. 
To minimize any bias, an open coding approach \cite{corbin1990grounded} was adapted which resulted in generating 42 codes reviewed and refined by the research team.
Two of the authors performed six rounds of pair coding to reach a shared understanding before individually coding the remaining interview scripts. 
During pair coding, the Cohen's Kappa \cite{landis1977measurement} were 0.51, 0.72, 0.73, 0.88, 0.76, and 0.76 which indicates we had moderate level of agreement.


% This process helped with better understanding the data and prepare a concrete codebook. 
% With the increase in number of codes, we classified the codes into further categories. 
% This helped us keep the codebook manageable and combined similar concepts together allowing us to reach saturation. 
% In total we identified 42 codes which was later categorized into four themes corresponding to our concept of product management and user feedback.
% Our findings comprise of the generated themes and quotes that are directly linked to these concepts. 

